Optimal Pricing Schemes in the Presence of Social Learning and Costly Reporting

A monopoly platform sells either a risky product (with unknown utility) or a safe product (with known utility) to agents who sequentially arrive and learn the utility of the risky product by the reporting of previous agents. It is costly for agents to report utility; hence the platform has to design both the prices and the reporting bonus to motivate the agents to explore and generate new information. By allowing sellers to set bonuses, we are essentially enabling them to dynamically control the supply of learning signals without significantly affecting the demand for the product. We characterize the optimal bonus and pricing schemes offered by the profit-maximizing platform. It turns out that the optimal scheme falls into one of four types: Full Coverage, Partial Coverage, Immediate Revelation, and Non-Bonus. In a model of exponential bandit, we find that there is a dynamical switch of the types along the learning trajectory. Although learning stops efficiently, information is revealed too slowly compared with the planner's optimal solution.

==> chapters/Bandit.tex <==
\section{Model Set Up}
\label{section_Imperfect_Learning}
There is a monopolistic seller offering two distinct products, denoted as $i=1,2$ (referred to as product 1 and 2 henceforth), to a sequence of risk-neutral agents in an infinite horizon, each with a lifetime of $\Delta\to0$ periods. In each period $\Delta$, a single agent is present. The production cost for each product is normalized to zero. The seller, being long-lived, aims to maximize its cumulative profit over time, while short-lived agents, having outside utility of 0, seek to maximize their expected utility within period $\D$ by selecting at most one product from the available options. Product 2 is considered a safe product with a known utility, while product 1 is categorized as a risky product, whose utility is unknown to both buyers and the seller. In line with previous literature, such as \cite{KRC2005}, we label product 2 as the "safe arm" and product 1 as the "risky arm". 

Choosing the safe arm results in a deterministic flow utility of $s>0$, while the utility of choosing the risky arm is modeled in the following bandit setting: purchasing the risky arm can yield either a lump-sum value $z$ (good news) or zero utility, contingent on a hidden state of the world unknown to both the seller and buyers. There are two states, denoted as good (G) or bad (B). In the good state, the arrival rate of realizing value $z$ follows an exponential distribution with parameter $\lambda$, i.e., the probability density function is $\lambda e^{-\lambda t}$. In the bad state, arm 1 always results in zero utility. After purchasing the risky arm, buyers can privately learn their own utility under the risky arm: either a lump-sum $z$ or zero utility. Since $z$ can only be achieved under the good state, we assert that this good news is conclusive. We introduce a crucial assumption \ref{assumption_meaningful} here to ensure our discussion is non-trivial; otherwise, the risky arm is dominated by the safe arm.
\begin{assumption}
	$g\equiv \lambda z>s>0$
	\label{assumption_meaningful}
\end{assumption}


After purchasing and privately observing their own utility, buyers can decide whether to disclose their news to the public (they cannot privately report to the seller to create information asymmetry). Due to their short-lived nature, there is no strategic incentive for them to lie or conceal information. However, the act of reporting itself incurs a cost, with each buyer having a private reporting cost $c_i$, independently and identically distributed according to the distribution function $H(\cdot)$ with support $[0,\bar{c}]$. For simplicity, we assume that $H(\cdot)$ is strictly increasing and has a smooth density function $h(\cdot)$. Moreover, we impose the following standard assumptions \ref{Inada} and \ref{assumption:monotone_beta} on the density function $h(\cdot)$ and virtue value  $\beta(x)=x+\frac{H(x)}{h(x)}$:
\begin{assumption}
\label{Inada}
The density function $h(\cdot)$ satisfies:
$\lim\limits_{x\to 0^+} h(x)>0$, and  $\lim\limits_{x\to c^-} h(x)>0$.
\footnote{A more general assumption for part 2 in Assumption \ref{Inada} is that there exists some order $p$ such that $\lim\limits_{x\to \bar c^-}h^{(p)}(x)\neq 0$ if $\lim\limits_{x\to \bar c^-}h^{(k)}(x)= 0,\forall k<p$.Here if $\lim\limits_{x\to \bar c^-}h(x)=0$, form L Hospital's Rule $\lambda(\bar c)=M+\bar c+\lim\limits_{x\to \bar c^-}\frac{H(x)-H^2(x)}{h(x)}=M+\bar c-\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ so if $\lim\limits_{x\to \bar c^-}h'(x)=0$ we can still get the same result by using  $\lim\limits_{x\to \bar c^-}h''(x)>0$ or so on. All we need is that the limit $\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ is convergent to zero hence as long as there exist some order $p$ such that $\lim\limits_{x\to \bar c^-}h^{(p)}(x)\neq 0$ if $\lim\limits_{x\to \bar c^-}h^{(k)}(x)= 0,\forall k<p$, which always exists unless $h(x)$ is constant in a neighborhood of $\bar c$. }
\end{assumption}

\begin{assumption}
$\beta(x)$ is continuously differentiable and 	$\beta'(x)$ is always positive.
 \label{assumption:monotone_beta}
\end{assumption}
Since, in our setting, $H(\cdot)$ has support with an upper bound of $\bar{c}$, a potential strategy is to employ the "Immediate Revelation" strategy, which involves setting a bonus of $\bar{c}$ to ensure that every buyer reports at the outset. We introduce assumption \ref{assumption_barc_large} to rule out this strategy. Further discussion on this matter will be presented in the appendix.
\begin{assumption}
	$\bar c>(\frac{\lambda}{r}+1)(g-s)$
 \label{assumption_barc_large}
\end{assumption}

We assume that each buyer can observe the entire purchasing and reporting history. This assumption allows us to concentrate on the pricing and report motivating problems. Although this assumption is evidently strong, we find that this situation is quite common in online markets, where potential consumers have full access to previous consumers' feedback. If consumers' reporting is privately observed by the seller, information design problems arise. This allows the seller to exploit a dynamic Bayesian persuasion strategy to motivate agents to purchase the risky arm (see \cite{kremer2014implementing}). 

In this scenario, society will collectively form a common belief regarding the probability that the state is good. Denote common purchasing and reporting history from past observations before time $t$ as
$\mathscr{F}(t)$, a natural state variable is the common belief $\alpha_t=\Pr(\theta=G|\mathscr{F}(t))$, which is the common posterior probability that $\theta=G$.

The seller's problem is to determine the pricing and bonus scheme. We permit the seller to commit to a contingent bonus scheme $\tilde{b}_t(\alpha_t)$ and pricing scheme $p_{1t}(\alpha_t), p_{2t}(\alpha_t)$ before the game starts. However, we do not allow bonuses to be contingent on the polarity of the feedback. This assumption rules out the trivial strategy of bribing for reputation.  It's also a reasonable assumption, since in most online purchasing platforms, the seller has no access to forbid consumers to provide negative feedback or complaints. Without loss of generality, we focus on pure strategies. 

The dynamic game hence consists of four components: the seller's pricing and bonus scheme, and the buyers' purchasing and reporting strategies. We limit our attention in Markovian strategies and equilibrium. We define the most general strategy here and refine them in section \ref{Section_preliminary_analysis}.

For the seller, the pricing scheme is a pair of measurable function $p_i:[0,1]\to \mathbb R$, where $i\in\{1,2\}$ stands for the price for the risky arm and safe arm separately. The bonus scheme is a measurable function $b:[0,1]\to [0,\bar c]$ where $b(\alpha_t)$ stands for the bonus for agent $t$ of reporting the utility after purchasing the risky arm. With this notation, the price and bonus is not dependent on time $t$ or reporting content.  Each buyer has demand of 1 product, the purchasing strategy $d_t(\alpha_t,p_{1t},p_{2t})$ determines which product to buy: $d_t: [0,1]\times \mathbb R^2 \to \{0,1,2\}$, where $d_t=0$ stands for no purchase. The reporting strategy $r_t(b_t,c_t)$ stands for whether agent $t$ would report, conditional on $d_t=1$: $r_t: \mathbb R^2 \to \{0,1\}$

\textbf{Timing.} We denote the agent residing in the interval $[t,t+\Delta)$ as agent $t$. $p_{1t}$ and $p_{2t}$ represent the prices for the risky arm and the safe arm at time $t$ respectively. If purchasing happens, the prices $p_{it}$ are paid at the beginning of this period. Moreover, if he decides to report when the bonus is $\tilde b_t$, he pays a deterministic flow cost $c_i$, and get bonus $\tilde b_t$ at the end of period $\Delta$\footnote{Hence the consumer has no incentive to report saying a good news earlier since the bonus is paid at the end of $\Delta$ no matter what he reports.}.
Thus, at time $t$, agent $t$ observes $p_{1t}$, $p_{2t}$, $\tilde{b}_t$, and the common belief $\alpha_t$ formed by the entire purchasing and reporting history before $t$.  Additionally, we consider a common exponential discount factor with discount factor $r$; that is, a payoff $v$ received at time $t$ generates a utility of $e^{-rt} v$ at time 0 both for the buyer and seller.

\textbf{Buyer's Surplus.} If agent $t$ purchases safe arm, he would have surplus \[\int_0^{\Delta} e^{-rt}s  dt-p_{2t} \]
If he chooses the risky arm, he may get the lump sum utility $z$ which may realize at any time $t$ with density $\lambda e^{-\lambda t}$ within $\Delta$. That is to say, if the consumer chooses risky arm, his expected surplus is
\[\int_0^{\Delta} e^{-rt}\lambda e^{-\lambda t} \alpha z dt-p_{1t} \] if he doesn't report. Otherwise, if he reports, the expected surplus is 
\[\int_0^{\Delta} e^{-rt}\lambda e^{-\lambda t} \alpha z  dt-p_{1t}-\int_{0}^{\Delta} e^{-rt} c_i dt+e^{-r\Delta} \tilde b_t\]
%During period $[t,t+\D)$ there will be one agent living, with demand of at most one product. If the agent purchases one of the products, the price is paid immediately (at $t$). If the agent reports, the bonus is paid at the end of the period (at $t+\D$). 
%Since the seller can always set $p_{2t}$ such that $\int_0^{\Delta} e^{-rt}s  dt-p_{2t}=\epsilon $ to guarantee a positive surplus, there are only three possible outcomes in potential optimal pricing schemes: selling a safe arm for sure, selling a risky arm for sure, and selling a risky arm with some probability. Assume within period $[t,t+\D)$ the price for the current seller is $p_{1t}$ and $p_{2t}$ with bonus $b_{t}$, then the stage payoff of the seller would be 

\textbf{Seller's Stage Payoff.} The seller's stage payoff within $[t,t+\D)$ depends on agent $t$'s actions $(d_t,r_t)$, which can be written as 
\[  \pi(\D,b_t,p_{1t},p_{2t})=\left\{
\begin{aligned}
	& p_{1t} & \text{ if } d_t=1,r_t=0 \\
	& p_{1t} - e^{-r\D} b_t & \text{ if } d_t=1,r_t=1\\
	& p_{2t} &\text{ if } d_t=2\\
	& 0 &\text{ if } d_t=0
\end{aligned} \right.
\label{equation_seller_payoffl} \]

\section{Model Analysis}
\label{section_Model_Analysis}
Our main result is Proposition \ref{optimal_switching_proposition} and \ref{proposition_speed}. Proposition \ref{optimal_switching_proposition} characterize the monopolist's optimal linkage between pricing and bonus setting, as well as the optimal switching between strategies and optimal stopping rules. Proposition \ref{proposition_speed} shows that the learning process led by the monopolist will terminate at the first best cutoff, while the learning speed is inefficiently low.  
\subsection{Seller's Strategy}
\label{Section_preliminary_analysis}
Within period $[t,t+\D)$, the seller can only sell at most one of the two products to agent $t$. Since he is the monopolist and buyer's outside utility is 0, the seller can always extract all the consumer surplus and sell whatever product he wants, by decreasing the target price with $\epsilon\to 0^+$ to create a positive surplus. For example, the seller can set $p_2(\alpha_t)=\frac{1-e^{-r\Delta}}{r}s$ and $p_1(\alpha_t)=\frac{\lambda(1-e^{-(r+\lambda)\Delta})}{\lambda+r}\alpha_t z-\epsilon$ to guide all buyers to buy risky arm. The seller can also $p_1=\frac{\lambda(1-e^{-(r+\lambda)\Delta})}{\lambda+r}\alpha_t z+\epsilon$ to guide all buyers who won't report to buy safe arm. 

Without loss of generality\footnote{For example, in \cite{bergemann2000experimentation}, safe product and risky product are provided by two sellers, and they consider the Bertrand competition to do tie breaking.}, we assume the seller will price fairly and consumers do tie breaking according to seller's policy $\ell(\alpha_t)$, where seller's policy $\ell:[0,1]\to \{1,2\}$ stands for which product he would sell to agents who doesn't report. 
In other words, we always set
\begin{equation}
\begin{aligned}
p_{1t}=&\int_0^{\Delta} e^{-rt}\lambda e^{-\lambda t} \alpha z dt=\frac{\lambda(1-e^{-(r+\lambda)\Delta})}{\lambda+r}\alpha z\\
        p_{2t}=&\int_0^{\Delta} e^{-rt}s  dt=\frac{1-e^{-r\Delta}}{r}s
    \label{price}
\end{aligned}
    \tag{Fair Pricing}
\end{equation}
and allows the seller to implement a common belief contingent bonus scheme $b_t(\alpha_t)$ and selling policy $\ell(\alpha_t)$. If the seller sets $\ell(\alpha_t)=2$ in the interval $[t_1,t_2]$, we can expect that, along the equilibrium path, almost all agents will opt for the safe arm, with only a fraction choosing the risky arm and submitting a report. Therefore, we label the case where $\ell(\alpha_t)=1$ as "promoting the risky arm" and $\ell(\alpha_t)=2$ as "promoting the safe arm" for simplicity. In general, there are four possible combinations of this selling policy and bonus scheme, as shown in Table \ref{table_strategy}. 

In the left of our analysis, we would define the seller's strategy as a combination of promoting policy $\ell:[0,1]\to \{1,2\}$ and bonus scheme $b:[0,1]\to \mathbb R$. The buyers would do tie breaking in favor of seller's promoting policy, and conditional on $\ell_t=1$, the buyer has reporting strategies $r_t:[0,\bar c]\to \{0,1\}$.

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}\hline
         &promoting risky arm &promoting safe arm \\\hline
         $\bar c>b_t>0$& Full Coverage & Partial Coverage\\ \hline
         $b_t=0$& Non Bonus & Safe Arm\\ \hline
    \end{tabular}
    \caption{$2\times 2$ strategies}
    \label{table_strategy}
\end{table}

\iffalse
\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|c|}\hline
         &promoting risky arm &promoting safe arm \\\hline
         $\bar c=b_t$ &\multicolumn{2}{|c|}{Immediate Revelation}
         \\\hline
         $\bar c>b_t>0$& Full Coverage & Partial Coverage\\ \hline
         $b_t=0$& Non Bonus & Safe Arm\\ \hline
    \end{tabular}
    \caption{$2\times 2$ strategies}
    \label{table_strategy}
\end{table}
\fi

By setting $b_t=0$, the selling policy uniquely determines the outcome. If the seller is promoting risky/safe arm, for sure the current agent $t$ will purchase the risky/safe arm. And there will be no learning because of no reporting, so we denote these stage strategies as ``Non Bonus'' (NB) and ``Safe Arm'' (SA) separately. The stage payoff of using NB and SA are:
\[\pi_{\text{NB}}(\D,b_t=0)=p_{1t}, \pi_{\text{SA}}(\D,b_t=0)=p_{2t}\]

By setting some $b_t>0$ and mainly selling risky arm, the seller has some probability to motivate the current agent to report, otherwise the current agent purchases the risky arm and not report. In this case, the seller uses risky arm to fully cover the market demand, hence we denote this strategy as ``Full Coverage'' (FC). Under Full Coverage, the agent with reporting cost $c_i$ will purchase the risky arm for sure and report if and only if 
\begin{equation}
    e^{-r\Delta}\tilde b_t-\int_0^{\Delta} e^{-rt } c_i dt\ge 0\label{report_condition}
\end{equation}
Hence by setting $\tilde b_t$ (or equivalently, setting $b_t\equiv \frac{r}{1-e^{-r\Delta}} \tilde b_t$), the ex-ante probability of successfully motivating the reporting is 
\[\pr(\text{report})=H(\frac{e^{-r\Delta}r}{1-e^{-r\Delta}} \tilde b_t)\equiv H(e^{-r\Delta} b_t)\]
Hence for the seller the immediate surplus is then 
\begin{equation}
\begin{aligned}
        \pi_{\text{FC}}(\Delta,b_t) &=p_{1t}-e^{-r\Delta}\tilde b_t\pr(\text{report}) \\&= \frac{\lambda}{r+\lambda} (1-e^{-(r+\lambda)\Delta})\alpha z -H(e^{-r\Delta}b_t) b_t\frac{1-e^{-r\Delta}}{r} e^{-r\Delta}
\end{aligned}
    \label{pi_FC_Delta}
\end{equation}

If the seller is mainly selling safe arm, then positive bonus may affect market demand. If the current agent has reporting cost $c_i$ and 
\begin{equation}
    \int_0^{\Delta} e^{-rt}\lambda e^{-\lambda t} \alpha z  dt-p_{1t}-\int_{0}^{\Delta} e^{-rt} c_i dt+e^{-r\Delta} \tilde b_t\ge \int_0^{\Delta} e^{-rt}s  dt-p_{2t} 
    \label{report_condition_PC}
\end{equation}
the current agent will purchase the risky arm and report  for sure. Otherwise he will purchase the safe arm in favor of partial coverage policy. Hence on the equilibrium path, all agents who doesn't report would purchase the safe arm, while those who purchases the risky arm would report for sure.  We call this strategy ``Partial Coverage'' (PC) in the sense that the seller is still learning the quality of risky arm, but only using it partially covering the market demand. 
The simplified expression of \eqref{report_condition_PC},  incorporating pricing and tie-breaking, leads to the same condition as \eqref{report_condition}. This indicates that, given an identical bonus scheme, agents who would report under Full Coverage will do so if and only if they would also report under Partial Coverage. So the probability of motivating the current agent to report would be the same.
Hence we can get
\begin{equation}
    \pi_{\text{PC}}(\Delta,b_t)=\pr(\text{report}) [p_{1t}-e^{-r\Delta}\tilde b_{t}] +[1-\pr(\text{report})] p_{2t}
    \label{pi_PC_Delta}
\end{equation}





\subsection{Seller's Value Function}
If it's already known that the state is good, value function of keeping selling $R_1$ will be:
\[
\tilde V=\int_0^{\Delta} e^{-rt} (\lambda e^{-\lambda t})z dt+e^{-r\Delta}\tilde V
\]
Let $\Delta \to 0$ we can get $\tilde V=\frac{\lambda z}{r}$. Similarly, keeping selling $R_2$ leads to payoff $\tilde U=\frac{s}{r}$, which is the value function of using Safe Arm strategy. With the same logic, the value function of using Non Bonus strategy should be $\frac{\alpha \lambda z}{r}$.

%The state variables of the seller is his belief (which is also the common belief that holds for buyers) of the possibility that the state is good. At time $t$ with belief $\alpha\circ \theta_G+(1-\alpha)\circ \theta_B$ the platform can choose one possible strategy $L$ from the set $\{$ NB(Non Bonus), SA(Safe Arm), FC(Full Coverage), PC(Partial Coverage) $\}$ which affects his value function by affecting immediate payoff (which item will be sold) and can set a bonus $b$ which influences the value function by affecting the probability of belief updating. 

%\red{In this case, it's obvious that the monopolist should use a cutoff strategy: when $\alpha= 0$ there is no Bayesian updating hence the monopolist will always use SA, and when $\alpha=1$, there is no need to do any test, hence with assumption  \ref{assumption_meaningful} the platform should use NB. Since SA (NB) can be achieved from PC(FC) by setting non bonus, we know that the monopolist is actually using a cutoff strategy: when $\alpha$ is higher, he is more likely to use FC and NB, and less likely to use SA or PC. Moreover, if the belief $\alpha$ is higher, the value function should always be (weakly) higher, since even though we use the same strategy, the immediate payoff would always increase if there is positive probability to sell the risky arm. Our question is how to design the optimal switching among these strategies.}

\iffalse
As we have mentioned, we always have
\[p_{2t}= \frac{s(1-e^{-r\Delta})}{r}\]
and 
\[p_{1t}=\frac{\lambda}{r+\lambda} (1-e^{-(r+\lambda)\Delta}) \alpha z\]
and consumers do tie breaking in favor of sellers' policy.


Under Full Coverage, the agent with reporting cost $c_i$ will purchase the risky arm and report for sure if and only if 
\[e^{-r\Delta}\tilde b_t-\int_0^{\Delta} e^{-rt } c_i dt\ge 0\]
\fi

Plug $\D\to0$ in equation \ref{pi_FC_Delta} and \ref{pi_PC_Delta}, we can get
\begin{equation}
    \lim_{\Delta\to 0} \frac{\pi_{\text{FC}}(\Delta,b_t)}{\Delta} = \lambda \alpha z-H(b_t)b_t
    \label{pi_fc}
\end{equation}
and 
\begin{equation}
     \lim\limits_{\Delta\to 0}\frac{\pi_{\text{PC}}(\Delta,b_t)}{\Delta}
    = H(b_t) [\lambda\alpha z-b_t] +[1-H(b_t)] s
    \label{pi_pc}
\end{equation}


As a conclusion of equation \eqref{pi_fc} and \eqref{pi_pc}, let $\pi_{L}(\Delta,b_t)$ stands for seller's expectation of immediate net profit within period $\Delta$ using strategy $L\in \{\text{FC,PC,NB,SA}\}$. If seller's policy at time $t$ is $(L,b_t)$ then the period profit fits
\begin{equation}
    \lim_{\Delta\to0}\frac{\pi_{L} (\Delta,b_t)}{\Delta}=\left\{
\begin{aligned}
	&\lambda \alpha z-H(b_t)b_t & \text{ if } L=\text{FC}\\
	& H(b_t) [\lambda \alpha z-b_t] +[1-H(b_t)] s & \text{ if } L=\text{PC}\\
	& \lambda \alpha z &\text{ if } L=\text{NB}\\
	& s &\text{ if } L=\text{SA}
\end{aligned} \right.
\label{equation_pi_1l}
\end{equation}
And the probability of reporting the utility of purchasing risky arm is
\[P_L(b_t) = \lim_{\Delta\to0} P_L(\Delta, b_t)=\left\{
\begin{aligned}
	&H(b_t)& \text{ if } L=\text{FC or PC}\\
	&0 &\text{ if } L=\text{NB or SA}
\end{aligned} \right.\]


Hence the seller's value function $\Pi(\cdot)$ follows the dynamic process:
\begin{equation}
    \Pi(\alpha)=\max\limits_{L,b} \pi_{L} (\Delta,b_t)+P_L(\Delta, b)e^{-r\Delta}\gamma(\alpha,\Delta) \Pi(\alpha')+
    P_L(\Delta, b) e^{-r\Delta}(1-\gamma(\alpha,\Delta)) \tilde V
    +(1-P_L(\Delta, b))e^{-r\Delta}\Pi(\alpha)
    \label{equation_max}
\end{equation}
where \[\gamma(\alpha,\Delta)=1-\alpha(1-e^{-\lambda \Delta})\] stands for the probability that in time period $\Delta$ the current agent reports a zero utility and then leads to belief updating to $\alpha'$, and  $1-\gamma(\alpha,\Delta)$ stands for the probability that within $\Delta$ the agent reports a utility $z$ which makes the common belief jump to 1 immediately. 
$P_L(\Delta,b)=\pr(\text{report})$ stands for the probability of motivating the current agent to report successfully under strategy $L$. The common belief will follow the Bayesian updating rule
\[
\alpha'=\frac{\alpha e^{-\lambda \Delta}}{\alpha e^{-\lambda \Delta}+1-\alpha}
\]


\iffalse
\[=\left\{
\begin{aligned}
	&[\frac{\int_0^{\Delta}re^{-rt}\lambda e^{-\lambda t} \alpha z dt}{(1-e^{-r\Delta})}- H(b)b](1-e^{-r\Delta}) & \text{ if } L=\text{Full Coverage}\\
	& (1-e^{-r\Delta}) [H(R) (p_1-b) +(1-H(R))s]dt& \text{ if } L=\text{Partial Coverage}\\
	& \int_0^{\Delta}re^{-rt}\lambda e^{-\lambda t} \alpha z dt &\text{ if } L=\text{Non Bonus}\\
	& s(1-e^{-r\Delta})&\text{ if } L=\text{Safe Arm}
\end{aligned} \right.\]
let $\Delta \to 0$ we can get:
\[\lim_{\Delta\to0}\frac{\pi_{L} (\Delta,b_t)}{\Delta}=\left\{
\begin{aligned}
	&\alpha z r \lambda -H(b)br& \text{ if } L=\text{Full Coverage}\\
	&[H(R) (p_1-b) +(1-H(R))s] r& \text{ if } L=\text{Partial Coverage}\\
	& \alpha z r \lambda &\text{ if } L=\text{Non Bonus}\\
	& rs&\text{ if } L=\text{Safe Arm}
\end{aligned} \right.\]
\fi

Let $\D\to 0$ (for more details, see Appendix \ref{appendix_proof_pre}), we can get $\Pi(\alpha)$ actually follows the ordinary differential equation based on equation (\ref{equation_max}):
\begin{equation}
    r \Pi(\alpha)=\max\limits_{L,b}\lim_{\Delta\to0}\frac{\pi_{L} (\Delta,b_t)}{\Delta}+P_L(b) \frac{\alpha \lambda^2 z }{r}-P_L(b)\alpha \lambda \Pi(\alpha)+P_L(b)(\alpha^2-\alpha)\lambda \Pi'(\alpha)
    \label{ODE_vf}
\end{equation}
In the left of this section, we characterize the optimal pricing and bonus scheme for the monopolist. To do so we first derive the optimal pricing and bonus scheme for the monopolist with bounded rationality, in the sense that he can use Full Coverage or Partial Coverage, with optimally stopping experiments and switching to Non Bonus and Safe Arm. As a main result here, Fact \ref{Fact_intersect} shows that these two value functions will intersect with a kink, hence the fully rational monopolist should optimally switching between Full Coverage and Partial Coverage, which is concluded in Proposition \ref{optimal_switching_proposition}. Then we characterize the optimal pricing and bonus scheme for a social planner for welfare analysis in terms of efficient termination and learning speed.
 
 \subsection{``Naive'' Monopolist}
 We first consider a simple scenario where the seller can only use one of two interior strategies: either $\FCO$ or $\PCO$. Additionally, the seller knows how to optimally switch between these interior strategies to the corner solution, namely, the Non-Bonus or Safe Arm strategy. We refer to this type of seller as a ``naive'' monopolist. In contrast, a fully rational seller who knows how to optimally switch among all strategies is termed an ``optimal switching monopolist''. Introducing the ``naive'' monopolist has its advantages, as analyzing its value function helps us study the possible patterns and directions for optimal switching.
 \iffalse
 The monopolist can optimally choose one of three possible strategies in Full Coverage, Partial Coverage, Safe Arm and Non Bonus based on the common belief, and it's quite intuitive that when the belief is high enough, the platform is willing to choose Full Coverage or Non Bonus, and when it's low , Safe Arm or Partial Coverage would be better. How to use Non Bonus and Safe Arm is quite clear: we know when the belief is extremely high (low), NB (SA) is optimal for sure. We also know that since NB (SA) can be considered as a corner solution of FC (PC), there should be a natural transition from FC (PC) to NB(SA). 
 
 The only question is whether the platform may choose Partial Coverage as a transition between Full Coverage and Safe Arm when the belief is decreasing, or switch from Full Coverage to Safe Arm directly (similarly between PC, FC and NB). The only way to answer this question is to compare the cutoff switching belief of switching from Full Coverage to Safe Arm and the cutoff switching belief of switching from Partial Coverage to Safe Arm. Hence, we should characterize the optimal strategy of ``Non optimal switching Monopolist'' or ``Naive Monopolist'', by which we mean the monopolist can only use part of the strategies and switch among them.
 \fi
 
 Firstly we consider ``Full Coverage Only'' monopolist (i.e. the seller can only use Full Coverage, Safe Arm or Non bonus). We denote $V(\alpha)$ as the value function of using Full Coverage. Combine equation (\ref{equation_pi_1l}) and (\ref{ODE_vf}), we can get 
 \begin{equation}
    r V(\alpha)=\max\limits_{b\in[0,\bar c]} \lambda \alpha z[1+H(b)\frac{\lambda}{r}]-H(b)b-H(b)\alpha \lambda V(\alpha)+H(b)(\alpha^2-\alpha)\lambda V'(\alpha)
    \label{result ode}
 \tag{FC-ODE}
\end{equation}
 which is a standard Bellman Equation. Followed by principal of optimality (\cite{SLP}), the value function $V(\cdot)$ is well-behaved, in the sense of continuous, differentiable, and convex. Since we only consider the possibility that the monopoly can stop doing Full Coverage experiments and switch to the Safe Arm or Non Bonus, the optimal stopping problem can be easily captured by smooth pasting condition. The following lemma describes the strategy under this setting:
 
 \begin{lemma}
 The ``Full Coverage Only'' monopolist uses a cutoff strategy:
 there exists $0<\underline \alpha_1<\hat \alpha_{FC}^{NB}<1$ such that he uses NB for $\alpha>\hat \alpha_{FC}^{NB}$, uses 
 SA for $\alpha<\underline \alpha_1$. Otherwise he uses FC and sets $b_t(\alpha)>0$ for $\underline \alpha_1\le \alpha \le \hat \alpha_{FC}^{NB}$. Denote $\underline b_1$ as the bonus at belief $\underline \alpha_1$, then $b_t(\alpha),V(\alpha)$ and $\underline \alpha_1,\underline b_1$ fit the following relationships:
 	\begin{enumerate}
 		\item 	First order condition: \[
 		\beta(b)=\frac{\alpha z \lambda^2 }{r}+(\alpha^2-\alpha)\lambda V'(\alpha)-\alpha\lambda V(\alpha)
 		\]
 		\item Bellman equation: \[
 		rV(\alpha)=\alpha z \lambda+\frac{H^2(b)}{h(b)}
 		\]
 		\item Optimal Stopping: \[\left\{
 		\begin{aligned}
 			& \beta(\underline b_1)=\frac{\underline \alpha_1  \lambda}{r} (z\lambda-s) \\
 			& s =\underline \alpha_1  z \lambda+ \frac{H^2(\underline b_1)}{h(\underline b_1)}
 		\end{aligned} \right.\]
 		\item Monotonically Decreasing: $b(\alpha)$ is monotonically decreasing with respect to $\alpha$. 
 	\end{enumerate}
  \label{fconly_lemma}
 \end{lemma}
 
Lemma \ref{fconly_lemma} claims that the monopolist is less willing to motivate agents' learning when the common belief is higher. Intuitively, there are two powers affecting bonus setting. When the belief is higher, the monopolist would think it's more possible to jump to 1 and hence get higher further profit, which provides high incentive to set high bonus (exploration). However, if the belief is already high enough, the seller takes advantage of high common belief, hence setting high bonus may increase the risk that the common belief drops under reporting, which hurts the future profit (exploitation). Lemma \ref{fconly_lemma} shows the latter power overcomes the first one when $\alpha$ is in the area that using Full Coverage is optimal. Actually as we will see later, the first concern can be solved by using PC. A natural result is
 \[s>\underline{\alpha_1} z \lambda\]
 which means the $\FCO$ monopolist would like to encourage agents to test the risky arm even when it yields lower expected utility than safe arm. That's the natural result of leading a social learning process, even though the monopolist can not optimally switch between all potential strategies. In the formal model, the seller may switch from FC to PC (instead of SA), which will be discussed in section \ref{section_optimal_switching}.
 
 Last but not least, we should emphasis the possibility of using Non Bonus. From interior solution got from part 1 in Lemma \ref{fconly_lemma}, Full Coverage will generate zero bonus when 
 \[\frac{\alpha z \lambda^2}{r} +(\alpha^2-\alpha)\lambda V'(\alpha)-\alpha\lambda V(\alpha)\le 0\]
 Combined with part 2 in Lemma \ref{fconly_lemma},it's equivalent (in the interior solution part) to 
 \begin{equation}
     \alpha> \hat\alpha^{NB}_{FC}\footnote{Here we use $\hat\alpha^{NB}_{FC}$ since it's not the true switching cutoff for the optimal switching monopolist, since the value function for the optimal switching monopolist has the different boundary condition, even though they fit the same relationship between $V'$ and $V$ mentioned in \ref{fconly_lemma}.}
     \label{Full Coverage Non Bonus}
 \end{equation}

 where $ \hat\alpha^{NB}_{FC}$ is the solution of $V(\alpha)=\frac{\alpha z \lambda}{r}$.   Equation  \ref{Full Coverage Non Bonus} shows that the monopolist would prefer Non Bonus to Full Coverage for $\forall \alpha\in(\hat\alpha^{NB}_{FC},1)$. In other words, if the temporary common belief $\alpha_t\in(\hat\alpha^{NB}_{FC},1)$, the monopolist will sell risky arm to each agent and won't motivate them to report the utility. As a result, the common belief would never change since no social signals are generated in this case. As mentioned before, the monopolist would set lower bonus when common belief is higher, given the common belief $\alpha<\hat\alpha^{NB}_{FC}$. In this period, the monopolist is motivating agents to do more experiments). Otherwise when $\alpha\in(\hat\alpha^{NB}_{FC},1)$, the monopolist would not set any belief though it's possible that some agents come and report a positive utility and push the common belief directly to 1, since he can sell the risky arm 
and take advantage of the pretty high common belief. 

 
 Secondly, we consider $\PCO$ monopolist setting. As before, the value function $U(\alpha)$ must fit the following ordinary differential equation:
 \[
 r U(\alpha)=\max_b H(b) (\lambda \alpha z-b) +[1-H(b)]s+H(b)\frac{\alpha \lambda^2 z}{r}+H(b)(\alpha^2-\alpha)\lambda U'(\alpha)-H(b)\alpha \lambda U(\alpha)
 \tag{PC-ODE}
 \]
 
 And the following lemma characterize the solution of optimal stopping problem of switching from $U(\cdot)$ to $\tilde U$

 \begin{lemma}
 The ``Partial Coverage Only'' monopolist uses a cutoff strategy:
 there exists $0<\underline \alpha_2<1$ such that he uses PC and sets $b_t(\alpha)>0$ for $\alpha>\underline \alpha_2$, and uses 
 SA for $\alpha<\underline \alpha_2$. Denote $\underline b_2$ as the bonus at belief $\underline \alpha_2$, then $b_t(\alpha),U(\alpha)$ and $\underline \alpha_2,\underline b_2$ fit the following relationships:
 	\begin{enumerate}
 		\item 	First order condition: 
            \[ \beta(b)=\lambda \alpha z -  s+\frac{\alpha z \lambda^2}{r}+(\alpha^2-\alpha)\lambda U'(\alpha)-\lambda \alpha U(\alpha)
 		\]
 		\item Bellman equation: \[
 		r U(\alpha)=s+\frac{H^2(b)}{h(b)} 
 		\]
 		\item Optimal Stopping: \[\left\{
 		\begin{aligned}
 			&\underline b_2=0\\
 			&\underline \alpha_2=\frac{rs}{\lambda(g-s)+rg}
 		\end{aligned} \right.\]
 		\item Monotonically Increasing: $b(\alpha)$ is monotonically increasing with respect to $\alpha$. 
 	\end{enumerate}
  \label{pconly_lemma}
 \end{lemma}

 
A noticeable fact is that in Partial Coverage the net bonus $R$ is monotonically increasing with respect to $\alpha$, unlike Full Coverage. As a result, $\PCO$ will not optimally switch to Non Bonus, even though he is allowed in this setting. A more detailed discussion about this fact is illustrated in the Figure \ref{fig:pqplot} later. The other fact is that $\underline b_2=0$. We will see in section \ref{section_welfare} that this result will be the key force driving our main welfare analysis.
Lemma \ref{fconly_lemma} and \ref{pconly_lemma} together describe the value function of the Naive Monopolist. A quick illustration is in Figure \ref{wrong_fc_pc}.  
 \begin{figure}[H]
 	\centering  %图片全局居中
 	{\label{Fig.sub.1}
 	\includegraphics[width=0.5\textwidth]{figures/wrong_fcl_pcl_version5.jpg}}
 	\caption{Value Functions of the Naive Monopolist}
 	\label{wrong_fc_pc}
 \end{figure}
 
 

 

 \subsection{Optimal Switching Monopolist}
 \label{section_optimal_switching}

In this section we consider whether the fully rational monopolist should switch from Full Coverage into Partial Coverage, or directly into Safe Arm when the belief is decreasing. From Figure \ref{wrong_fc_pc} we can see a kink for value function for Full Coverage only monopolist and Partial Coverage only monopolist. We have a claim to show it's true in general.
\begin{fact}
    The value function for $\FCO$ monopolist and  $\PCO$ monopolist always intersect.
    \label{Fact_intersect}
\end{fact}
\begin{proof}
    Obviously  from lemma \ref{fconly_lemma} we know
    $rs=r\underline\alpha_1 g+rH(\underline b_1)[\beta(\underline b_1)-\underline b_1]$, so
\[\begin{aligned}
    rs&=\underline\alpha_1gr+\underline\alpha_1\lambda(g-s)H(\underline b_1)-r\underline b_1H(\underline b_1)\\
    &<\underline\alpha_1gr+\underline\alpha_1\lambda(g-s)
\end{aligned}
\]
while from lemma \ref{pconly_lemma} we know 
\[rs=\underline\alpha_2 gr+\underline\alpha_2\lambda(g-s)\]
assumption \ref{assumption_meaningful} guarantees $g>s$, hence we always have
	\[\underline \alpha_1>\underline \alpha_2\]
 
Combined with convexity, we know $V(\alpha)$ and $U(\alpha)$ is single-crossing in non trivial part.
\end{proof}

 In other words, there should be an optimal switching between FC and PC. And PC should optimally switching to Safe Arm. Hence we denote
\[\alpha^{PC}_{SA}=\underline \alpha_2\]
Which shows that the ODE (together with boundary condition) described in lemma \ref{pconly_lemma} pin down the value function of optimal switching monopolist using PC. 

We denote the switching belief as $\alpha^{PC}_{FC}$. Then the optimal switching condition (boundary condition for the ODE described in lemma \ref{fconly_lemma} ) should be changed as
\begin{equation}
V(\alpha_{PC}^{FC})=U(\alpha_{PC}^{FC}),V'(\alpha_{PC}^{FC})=U'(\alpha_{PC}^{FC})
	\label{smooth past}
\end{equation}

 An intuitive explanation may be that Partial Coverage here can be understood as a mixed strategy of using Full Coverage and selling safe arm. A numerical illustration can be found in comparison between figure \ref{wrong_fc_pc} and figure \ref{fig:correct_fcl_pcl}, where it looks as if we try to connect $V(\alpha)$ and $U(\alpha)$ smoothly when the first optimal switching occurs. More over we can prove:
\[\alpha_{PC}^{FC}=\frac{s}{z\lambda}\]
where the right hand side is nothing but the cut-off of the myopic monopolist (i.e. the monopolist who can only consider the present profit instead of the value function including discounted future profits). Base on Lemma \ref{fconly_lemma}, \ref{pconly_lemma} and equation \ref{smooth past}, we use the following proposition to state the optimal strategy of the monopolist completely.

Moreover, we can also prove $\alpha_{FC}^{NB}>\alpha_{PC}^{FC}$, since we have $b>0$ at $\alpha_{PC}^{FC}$, and $b=0$ at $\alpha_{FC}^{NB}$.
\begin{proposition}
There exists cutoffs $0<\alpha_{SA}^{PC}<\alpha_{PC}^{FC}<\alpha_{FC}^{NB}<1$, where $\alpha_{SA}^{PC}=\frac{sr}{\lambda(g-s-zr)},\alpha_{PC}^{FC}=\frac{s}{\lambda z}, \text{ and } \alpha_{PC}^{FC} \text{ solves } V(x)=xz\lambda $, such that:
\begin{itemize}
     \item if $0<\alpha< \alpha_{SA}^{PC}$, the social planner would use Safe Arm.
     \item if $\alpha_{SA}^{PC}<\alpha<\alpha_{PC}^{FC}$, the social planner would use Partial Coverage.
     \item if $\alpha_{PC}^{FC}<\alpha<\alpha_{FC}^{NB}$, the social planner would use Full Coverage.
     \item if $\alpha_{FC}^{NB}<\alpha<1$, the social planner would use Non Bonus.
 \end{itemize}
\label{optimal_switching_proposition}
\end{proposition}
To illustrate our results, a numeric example is provided whose details can be found in Appendix \ref{appendix_numeric}.  Figure \ref{fig:correct_fcl_pcl} is a numeric result based on the same parameters in Figure \ref{wrong_fc_pc}.  The horizontal axis stands for $\alpha$ and the vertical axis stands for the value function. 

%Moreover, we should notice that the optimal switching belief between FC and PC is $\alpha_{PC}^{FC}=\frac{s}{z\lambda}$, which is the exact belief when the one shot payoff of selling the risky arm, $\alpha z\lambda$ is equal to the one shot payoff of selling the safe arm $s$. According to our bullet points 4 in Lemmas \ref{fconly_lemma} and \ref{pconly_lemma}, we know the optimal reporting bonus should be monotonically decreasing with respect to $\alpha$ under FC but increasing under PC. This is to say, at the switching belief $\alpha_{PC}^{FC}$, the reporting bonus attaches the local maximum. Intuitively, the value of information attaches the maximum when the belief is at its vaguest state. An illustration is Figure \ref{fig:pqplot}.

\begin{figure}[H]
\centering  %图片全局居中
\includegraphics[width=0.5\textwidth]{figures/correct_fcl_pcl_r2_version5.jpg}
\caption{Optimal Switching Monopolist}
\label{fig:correct_fcl_pcl}
\end{figure}


\subsection{Welfare Analysis}
\label{section_welfare}
\subsubsection{Social planner's problem : a mechanism design way}
We consider such a setting, where a social planner, commits an allocation rule $p(\alpha,\cdot)$, a transfer rule $\tilde t(\alpha,\cdot)$ (or equivalently, denote $t(\alpha,\tilde c)=\lim\limits_{\Delta\to 0 }\frac{\tilde t(\alpha,\tilde c)}{\Delta}$) and a reporting rule $q(\alpha,\cdot)$.  Then the current agent with true cost $c_i$ arrives and reports his own reporting cost $\tilde c_i$, and the social planner will allocate and enforce transfer and reporting based on $\alpha$ and $\tilde c_i$. Reporting, allocation and transfer will be realised at the beginning of period $[t,t+\D)$, and the report (if any) will happen at the end.

Allocation rule stands for the probability of delivering the risky arm to the current agent, and probability $1-p(\alpha,\cdot)$ to deliver the safe arm. The agent will be charged a transfer $t(\alpha,\tilde c_i)$ no matter which arm is purchased. Then conditional on  getting the risky arm, the agent has probability $q(\alpha,\tilde c)$ to be obliged to report the true utility and $1-q(\alpha,\tilde c)$ to do nothing. Then for the agent with true cost $c_i$, reporting $\tilde c$ leads to utility\footnote{In duration $\Delta$, the agents' utility can be written as $\mathbb E(Surplus)=-\tilde t(\alpha,\tilde c)+p(\alpha,\tilde c) \int_0^{\Delta} \lambda e^{-\lambda t}e^{-rt}\alpha z dt-p(\alpha,\tilde c) q(\alpha,\tilde c) \int_0^{\Delta}e^{-rt} c dt+[1-p(\alpha,\tilde c) ] \int_0^{\Delta} s e^{-rt} dt$ . We denote $U(c,\tilde c,\alpha)=\lim\limits_{\Delta\to 0 }\frac{\mathbb E(Surplus)}{\Delta}$ . }
\[U(c,\tilde c,\alpha)=-t(\alpha,\tilde c)+p(\alpha,\tilde c)[\alpha z \lambda - q(\alpha,\tilde c) c]+(1-p(\alpha,\tilde c))s\]
and IC constraint hence requires 
\[c\in \arg\max_{\tilde c} U(c,\tilde c,\alpha)\]

For the social planner, in period $\Delta$, if the current agent reports $\tilde c$ (we use $c$ to replace $\tilde c$ since in equilibrium we have truthfully reporting), his immediate gain from total social surplus, should be 
\begin{equation}
\tilde \pi(\triangle,c)=p(\alpha, c) \int_0^{\Delta} \lambda e^{-\lambda t} e^{-rt} \alpha z dt -p(\alpha, c)q(\alpha, c) \int_0^{\Delta} e^{-rt}c dt +\int_0^{\Delta}e^{-rt}[1-p(\alpha, c)]sdt\label{equation_social}
\end{equation}

Then we define the value function, which is based on $\alpha$ only and stands for the expected total utility when holding belief $\alpha$. According to our definition of $\tilde \pi(\Delta,c)$, we have (The formation details can be found in Appendix \ref{Section_formation_social_planner})
\[W(\alpha)=\mathbb E_c(\pi(\alpha,c))=\int_c \pi(\alpha,c)dH(c)\]

Then we apply the operator $\int_c \cdot dH(c)$ for equation (\ref{equation_social}), (i.e. take the expectation with respect to $c$) for both sides, we can execute the limit calculation by using L'Hospital's Rule:
\[[r+\lambda \alpha \mathbb E(pq)]W(\alpha)=r\lambda \alpha z \mathbb E(p)+[1-\mathbb E(p)] sr-r\mathbb E(pqc)+\lambda^2 z\alpha \mathbb E(pq)+(\alpha^2-\alpha)\lambda W'(\alpha)\mathbb E(pq)\]

And the social planner should set the optimal $(t,q,p)$ to maximize $W(\alpha)$. Proposition \ref{proposition_socialplanner} describes the optimal strategy for the social planner. Denote $B(\alpha)\equiv \frac{\alpha\lambda^2 z}{r}+(\alpha^2-\alpha)\lambda W'(\alpha)-\lambda \alpha W(\alpha)$, $C_1(\alpha)\equiv\frac{B(\alpha)+\lambda z \alpha -s}{\lambda}$ and $C_2(\alpha)\equiv\frac{B(\alpha)}{\lambda}$, then we have: 
\begin{proposition}
    There exists optimal mechanism $(p,q,t)$ to guarantee that every agent will truthfully report their cost. There exists cutoff $\bar \alpha_{SA}^{PC}$, $\bar \alpha_{PC}^{FC}$ and $\bar \alpha_{FC}^{NB}$ and cutoff $C_1(\alpha)$ and $C_2(\alpha)$ for agents' cost,  such that:
 \begin{itemize}
     \item if $0<\alpha<\bar \alpha_{SA}^{PC}$, the social planner would set $p=q=0$ (i.e. using Safe Arm).
     \item if $\bar \alpha_{SA}^{PC}<\alpha<\bar \alpha_{PC}^{FC}$, the social planner would set $q=1$ for sure and $p=1$ if $c<C_1(\alpha)$ (i.e. using Partial Coverage).
     \item if $\bar \alpha_{PC}^{FC}<\alpha<\bar \alpha_{FC}^{NB}$, the social planner would set $p=1$ for sure and $q=1$ if $c<C_2(\alpha)$ (i.e. using Full Coverage).
     \item if $\bar \alpha_{FC}^{NB}<\alpha<1$, the social planner would set $p=1,q=0$ for sure (i.e. using Non Bonus).
 \end{itemize}
 \label{proposition_socialplanner}
\end{proposition}

Above proposition \ref{proposition_socialplanner} shows that social planner's decision is also based on the same optimal switching.  Like before, the social planner is more likely to use Full Coverage when the common belief is high (and Non Bonus is the common belief is even higher), use Safe Arm when belief is low, and use Partial Coverage as a transition when belief is moderate. More specifically, when $\alpha>\bar \alpha_{PC}^{FC}$, $p=1$ for sure, which means the social planner will always ask the agent to try the risky arm and report if the current agent is with a low enough $c$ such that $q=1$, which is like using Full Coverage.  Otherwise when $\bar \alpha_{SA}^{PC}<\alpha<\bar \alpha_{PC}^{FC}$, $p$ is possible to be zero when $c$ is large. The social planner will only ask agents with low enough costs to test the risky arm, hence it's equivalent to Partial Coverage. What’s still important here is that the once the social planner ask an agent to test the risky arm, the agent will be obliged to report(for more details please check Appendix \ref{Proof_proposition_socialplanner}). In a more intuitive way, these agents whose reporting cost is small enough to let $p=1$ for them are asked to use risky arm to explore rather than exploit the risky arm since myopically safe arm is better. When $\alpha<\bar \alpha_{SA}^{PC}$, the social planner will set $p=0$ for sure, which means the information aggregation is terminated, and the social planner sets Safe Arm. As before we can still characterize $W(\alpha)$ via a ODE system, which can be found in section \ref{proof_social_planner_optimization}.

A key message is that the switching cutoff belief is irrelevant with the decision maker. To be more specific:
\begin{enumerate}
	\item The social planner will switch to Partial Coverage at the same belief cutoff as the monopolist. At the cutoff belief, the decision maker should feel indifferent myopically between safe arm and risky arm, since the reporting probability is continuous at this cutoff. 
	\item The social planner will stop at the same belief cutoff as the monopolist. Though surprising at the first sight, actually the switching condition guarantees this equivalence. $\underline \alpha_2$ actually stands for the switching belief between Partial Coverage and Non Bonus, at which in the long run the decision maker feels indifferent between doing more experiment or not. One more experiment is of no value when the common belief is low enough, and it's irrelevant with the cost of experiment. Intuitively speaking, because of the existence of Partial Coverage, if the information is valuable for the social planner, it's also valuable for the monopolist since the monopolist can always set a low enough bonus and use Partial Coverage, and keep waiting until agents with low enough cost arrive, try the risky arm and report. 
\end{enumerate}



\subsubsection{Comparison of social planner's strategy and monopolist's strategy}
\label{section_comparison}
We measure the efficiency of the learning process led by the monopolist in two ways. Firstly, will the monopolist stop experiments at a higher belief? And secondly, will the monopolist attach the termination sooner than the social planner? The following proposition answers the first question:

\begin{proposition}
	  At any belief, the social planner will do experiments with (weakly) higher probability. As a result  $\bar \alpha_{FC}^{NB}> \alpha_{FC}^{NB}$. Moreover, the social planner will switch from Full Coverage to Partial Coverage, and switch from Partial Coverage and Non Bonus at the same believes as the monopolist (i.e. $\bar \alpha_{SA}^{PC}= \alpha_{SA}^{PC}$, and $\bar \alpha_{PC}^{FC} = \alpha_{PC}^{FC}$).
   \label{proposition_speed}
\end{proposition}



Proposition \ref{proposition_speed} that the monopolist's willingness do experiments is less than the social planner, hence every stage there is lower probability to report. Since the social planner bears less cost than the monopolist ($\mathbb E(c|c<b)<b$), a quick thought should be that the social planner will encourage agents with higher reporting cost to report than the monopolist. In other words, the learning speed of the social planner should be higher. ``Learning speed'' actually means reporting probability in our model (instead of arrival rate $\lambda$). We should realize that here social planner can naturally do better since he can design the reporting probability on $\alpha,c$ while the monopolist can only set it on $\alpha$. 
\begin{figure}[H]
\centering  %图片全局居中
\includegraphics[width=0.5\textwidth]{figures/pqplot_v4}
\caption{Mechanisms Comparison }
\label{fig:pqplot}
\end{figure}

A further illustration is in Figure \ref{fig:pqplot}. Both using Full Coverage, when the current agent's reporting cost $c$ is lower than the red solid line, the social planner is willing to set $p=q=1$, while the monopolist is only willing to set $p=q=1$ when  $c$ is lower than the red dotted line. We can find the monopolist will have lower probability to do experiments than the social planner.
Similarly, blue lines stands for the Partial Coverage, and our observations still hold. 


\subsubsection{Social Surplus under Monopolist's Setting}
Section \ref{section_comparison} demonstrates that the learning speed under the monopolist setting is consistently lower than that under the social planner. A subsequent question arises: does the slower learning speed lead to inefficiency? To address this inquiry, we require the value function of social surplus under the monopolist setting. Intuitively, the monopolist sets a lower bonus primarily to avoid incurring reporting costs. Hence, a natural conjecture is that a lower learning speed aligns with inefficiency. In this section, we will substantiate this intuition (refer to Figure \ref{fig:newsocial}).


To calculate the social surplus under the monopolist setting, we first express the value function and payoff contingent on the current agent's cost $c$ and then take expectations (More details are in Appendix \ref{Social_Surplus_Monopolist}). Conditional on $c$, we denote $P_L(b)=\mathbb I(b>c)$ as whether the current agent would report and modify equation \eqref{equation_pi_1l} as
\begin{equation}
    \mathbb E_c\lim_{\Delta\to0}\frac{\pi_{L}(\Delta,c)}{\Delta}=\left\{
\begin{aligned}
	&\alpha z \lambda - H(b)\mathbb E(c|c<b)& \text{ if } L=\text{FC}\\
	&H(b) \lambda z \alpha-H(b)\mathbb E(c|c<b) +[1-H(b)]s& \text{ if } L=\text{PC}\\
	& s&\text{ if } L=\text{SA}\\
    & \alpha z  \lambda &\text{ if } L=\text{NB}
\end{aligned} \right.
\label{stage_value_function_social_surplus}
\end{equation}

\begin{figure}[H]
	\centering
	\includegraphics[width=0.7\linewidth]{figures/surplus3_r2_version5.jpg}
	\caption{Social Welfare Comparison}
	\label{fig:newsocial}
\end{figure}

Under the monopolist setting, the disparity between social surplus and producer surplus arises because the seller incurs a loss of $b_t>c_t$ when successfully motivating agent $t$ to report, whereas for the social surplus, the loss is $c_t$. As a natural consequence, the value function of social surplus is always weakly higher than the value function of producer surplus. Furthermore, they coincide when there is no reporting, i.e., when $\alpha>\alpha_{FC}^{NB}$ or $\alpha<\alpha_{SA}^{PC}$. In Figure \ref{fig:newsocial}, $\alpha_{FC}^{NB}$ represents the monopolist switching cutoff, at which the red dotted line intersects with the black solid line.

This discrepancy also extends to the social planner's setting. Thus, if the social planner optimally designs the mechanism to maximize social surplus, they can outperform the monopolist, resulting in a value function that is also weakly higher than the value function of social surplus under the monopolist setting. As illustrated in Figure \ref{fig:pqplot}, the social planner switches between Partial Coverage and Safe Arm at the same cutoff as the monopolist but shifts to Full Coverage from Non Bonus at a higher cutoff. We use $\alpha_{FC}^{*NB}$ to denote the social planner's switching cutoff. For $\alpha>\alpha_{FC}^{*NB}$—since both the social planner and monopolist don't conduct experiments—their value functions should be the same. That's why in Figure \ref{fig:newsocial} both the black line and red dotted line intersect with the blue solid line when $\alpha>\alpha_{FC}^{*NB}$. 

In conclusion, this comparison reveals that social surplus under the monopolist setting is weakly lower than that under the social planner setting, suggesting that the monopolist would lead an inefficient learning process. Even when both learning processes terminate at the same cutoff, a lower learning speed adversely affects social surplus.



\iffalse
We consider the following setting for our welfare analysis, where there is a social planner who can see the common belief about good state $\alpha$, based on which he decides whether to let the current agent to try the safe arm or the risky arm. Then the social planner can see the reporting cost of the current agent, $c_t$, and decide whether to let the current agent report his utility. In this setting, once the platform lets the current agent to try the safe arm, there is no chance that the agent is willing to use the risky arm and reveal its utility. In other words, the social planner can only use ``Full Coverage'' here. In this setting, it's obvious that social planner uses cut-off strategies to make both decisions: to let the agent try the risky arm if $\alpha$ is high enough; and to let the agent report his utility of risky arm if his cost is lower than a threshold $\omega$ which is dependent on $\alpha$. In other words, given the current agent $t$ is going to try the risky arm, he will report if  $c_t<\Omega(\alpha)$. It will cost $c_t$ for the social welfare finally, but at the stage when the social planner makes his decisions, he can only expect the cost will happen conditional on $c_t<\Omega(\alpha)$. For this reason, we denote $\tilde \Omega=\mathbb E(c|c<\Omega)=\int_0^{\Omega}xdH(x)$ for the expected cost. In this setting, we drop the subscript and use $P(b)$ and $\pi_2$ for probability of motivating the current agent to report successfully and the immediate social surplus got from the current agent, then
we have $P(b)=H(\Omega)$ and $\pi_2=\int_0^{\Delta} re^{-rt}[\lambda e^{-\lambda t}\alpha z-\tilde\Omega H(\Omega)] dt$. We use $W(\alpha)$ for social planner's value function,  and similar to equation \ref{ODE_vf}, it fits the following ODE:
\[
    [r+H(\Omega)\alpha \lambda ] W(\alpha)=\alpha z \lambda r-H(\Omega)\tilde \Omega r+H(\Omega)(\alpha^2-\alpha)\lambda W'(\alpha)+H(\Omega)\alpha \lambda^2 z \tag{SP-ODE}
\]
And again the optimal switching problem here is when to switch from $W(\alpha)$ to $\tilde U$. The following lemma describes the solution:
\begin{lemma}
	Denote $\tilde \Omega =\int_0^{\Omega}xdH(x)$, then the social planner would let the agent to try the risky arm when $\alpha>\underline \alpha_4$, and would let the agent to report the utility of the risky arm when $c_t<\Omega(\alpha)$. Denote $\underline \Omega_4$ as the reporting cut-off at belief $\underline \alpha_4$, then $\Omega(\alpha),W(\alpha)$ and $\underline \alpha_4,\underline \Omega_4$ fit the following relationships:
	\begin{enumerate}
		\item 	First order condition:\[
	r[\tilde \Omega+H(\Omega)\Omega]=\alpha z \lambda^2+(\alpha^2-\alpha)\lambda W'(\alpha)-\alpha\lambda W(\alpha) 
\]
		\item Bellman equation: \[
	W(\alpha)=\alpha z \lambda+H^2(\Omega)\Omega
\]
		\item Optimal Stopping: \[\left\{
\begin{aligned}
	&\underline \Omega H(\underline \Omega)+\int_0^{\underline \Omega}xdH(x)=\lambda \underline{\alpha} \frac{\lambda z-s}{r}\\
	& s=\underline \alpha z\lambda+\underline \Omega H^2(\underline \Omega)
\end{aligned} \right.\]
	\item $\Omega(\alpha)$ is monotonically decreasing with respect to $\alpha$.
	\end{enumerate}
\end{lemma}

Compared with proposition 5.3, we can compare the value function of a Full Coverage only social planner, the value function of a Full Coverage only monopolist and the value function of a monopolist who can optimally switch among Full Coverage, Partial Coverage and selling safe arm. A numerical illustration is like figure \ref{fig:odevaluefunction} and from which there are two immediate observations from figure \ref{fig:odevaluefunction}:
\begin{enumerate}
	\item $W(\alpha)$ is always weakly higher than $V(\alpha)$, and $\underline\alpha_4<\underline\alpha_1$. Social planner has higher value function than Full Coverage monopolist since social planner has cheaper way to motivate report (it costs the expectation conditional on the cost is lower than the cutoff for the social planner, while it costs the cutoff for the monopolist). 
	\item $W(\alpha)$ is not always higher than $U(\alpha)$, and $\underline\alpha_4>\underline\alpha_2$. When the social planner has already stopped his experiments and begins to sell safe arm because of a low belief, the monopolist may still be experimenting using Partial Coverage, since it costs less to do experiments than Full Coverage, even social planner can do experiments in a cheaper way. 
\end{enumerate}

Our proposition 5.5 shows that these two observations does not rely on our numerical setting and describes our main results in welfare analysis:
\begin{proposition}
	We always have $\frac{s}{z\lambda}=\underline\alpha_3>\underline\alpha_1>\underline\alpha_4>\underline\alpha_2$
\end{proposition}
If the monopolist is myopic of whom learning values nothing, he can get $p_2=s$ by selling safe arm and get $p_1=\alpha z \lambda$ by selling the risky arm when the common belief is $\alpha$. Hence $\frac{s}{z\lambda}$ is just the belief for a myopic monopolist who feels indifferent between selling risky arm and safe arm. At $\underline \alpha_3$, the monopolist feels indifferent between selling the risky arm with Full Coverage or Partial Coverage since these two strategies have the same power to motivate experiments and the same expected price. This is an intuitive explanation of  $\frac{s}{z\lambda}=\underline\alpha_3$.
The fact $\frac{s}{z\lambda}>\underline\alpha_1$, as an echo of \cite{rothschild1974bandit}, shows the classic result that the monopolist may cherish the value of learning hence encourage more experiment than in myopic sense. 

The second inequality, $\underline\alpha_1>\underline\alpha_4$, shows that the social planner is more patient to do experiments than the monopolist, when they are only able to sell risky arms using Full Coverage. The value function of the social planner, $W(\alpha)$ is always higher than $V(\alpha)$, the value function of the Full Coverage only monopolist, not only because social planner costs less to do experiments, but also because social planner is hence more willing to do experiment with higher cutoff (i.e. $\Omega(\alpha)>b(\alpha)$), hence gains more value of information. In other words, if the monopolist can also only use Full Coverage strategy, the learning caused by the monopolist will be terminated inefficiently.

The third inequality shows that the monopolist may do experiments more efficiently than the social planner if the monopolist can use Partial Coverage strategy while the social planner can not, based on our setting. \textcolor{red}{is this Over-learning?} 
\begin{figure}[h]
	\centering
	\includegraphics[width=0.7\linewidth]{social}
	\caption{Comparison of Social Planner and Monopolist}
	\label{fig:odevaluefunction}
\end{figure}

Then we focus on how bonus scheme is affected by the belief in different settings.  
An illustration is in figure  \ref{fig:bonus} where we can find two main facts (notice that for Partial Coverage we use $R$ rather than $b$ in vertical axis):
\begin{enumerate}
	\item In Full Coverage strategies, no matter the decision maker is the monopolist or the social planner, the bonus is always lower when the common belief is higher. On the contrary, the bonus will be higher when the common belief is higher in Partial Coverage strategy. In Full Coverage, bonus reflects how much the decision maker values one more experiment only, unlike in Partial Coverage where bonus reflects not only the experiment value of the decision maker, but also the value difference between safe arm and risky arm. Because a higher bonus will guide the current agent to purchase risky arm with higher probability, the monopolist with Partial Coverage strategy is willing to set higher bonus when belief is high (hence the profit of selling risky arm is high).
	\item The social planner is willing to set higher bonus when using Full Coverage, but he will start setting zero bonus from a higher belief than the optimal switching monopolist because the social planner faces less cost than the monopolist when setting the same bonus.
\end{enumerate}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.5\linewidth]{bonus0323}
	\caption{Different bonus schemes}
	\label{fig:bonus}
\end{figure}
\fi


\subsection{Comparative Statics}
Here we do some comparative statics. We have discussed the effects of monopolist's behavior caused by discount rate $r$, relative utility $R_2$ , $\mathbb ER_1$ and $\mathbb \max \mathbb E\{R_1.R_2\}$. Here we add some new intuitions: how $\lambda$ (the perfect level of experiment) affects the monopolist's behavior in section \ref{comparative_lambda}, and how discount rate affects the social planner's behavior in section \ref{comparative_r}.  

\subsubsection{Comparative Statics for $\lambda$}
\label{comparative_lambda}
In this case we focus on discussing how the arrival rate $\lambda$ affects our results. Actually the larger arrival rate stands not only the risky arm is more attractive when the state is known to be good (since selling the risky arm leads to immediate profit $\alpha \lambda z$ ), but also the measure of the imperfect learning (since after purchasing the risky arm, there is probability $\alpha(1-e^{-\lambda \Delta})$ to get a positive feedback after an experiment with duration $\Delta$). So if we fix $s$, a larger $\lambda$ will make FC and NB more attractive hence we will see $\alpha_{SA}^{PC}$ and 
$\alpha_{PC}^{FC}$ will shrink to zero. A more meaningful way is to focus on the second power: how will the results change if the learning is ``less imperfect''. To do so we can re-define $s=\lambda z \rho$ where $\rho<1$ is a fixed constant who guarantees that the safe arm and risky arm is comparable in stage utility (i.e. to rule out the first effect). The intuition should be that if the learning is ``less imperfect'', then the seller will be more willing to do the experiment, hence we should expect a smaller $\alpha_{SA}^{PC}$ (and tends to 0 if $\lambda \to \infty$), and a larger $\alpha_{SA}^{PC}$ (and tends to 1 if $\lambda \to \infty$). The first intuition is easy to check since we have the analytical solution for $\alpha_{SA}^{PC}$. As for the $\alpha_{FC}^{NB}$, we have the following illustration Figure \ref{fig:lambda} by letting 
$\rho=0.5,r=0.5,z=7$ and we let $\lambda$ to grow from 0.2 to 2.

\begin{figure}[H]    
  \centering           
  \subfloat[$\lambda=0.3$]  
  {
\label{fig:subfig1}\includegraphics[width=0.4\textwidth]{figures/lambda03.jpg}
  }
  \subfloat[$\lambda=0.8$]
  {
\label{fig:subfig2}\includegraphics[width=0.4\textwidth]{figures/lambda08.jpg}
  }
  
  \subfloat[$\lambda=1$]
  {
\label{fig:subfig3}\includegraphics[width=0.4\textwidth]{figures/lambda10.jpg}
  }
  \subfloat[$\lambda=2$]
  {
\label{fig:subfig2}\includegraphics[width=0.4\textwidth]{figures/lambda20.jpg}
  }
  \caption{$\lambda$ Affects $\alpha_{FC}^{NB}$}    
  \label{fig:lambda}            
\end{figure}


\subsubsection{Comparative Statics for $r$}
\label{comparative_r}
We do comparative statics here with respect to  $r$, the discount factor of the decision maker. A direct idea is value functions should be monotonically decreasing with respect to the discount rate $r$. Moreover, with higher $r$, the decision maker will be less willing to do experiments, no matter in Monopolist case or Social Planner case. An illustration (take social surplus as an example) is like Figure \ref{fig:r}:

\begin{figure}[H]    
  \centering            
  \subfloat[$r=0.2$]  
  {
\label{fig:subfig1}\includegraphics[width=0.4\textwidth]{figures/r02.jpg}
  }
  \subfloat[$r=0.5$]
  {
\label{fig:subfig2}\includegraphics[width=0.4\textwidth]{figures/r05.jpg}
  }
  
  \subfloat[$r=0.9$]
  {
\label{fig:subfig3}\includegraphics[width=0.4\textwidth]{figures/r09.jpg}
  }
  \subfloat[$r=1.2$]
  {
\label{fig:subfig2}\includegraphics[width=0.4\textwidth]{figures/r12.jpg}
  }
  \caption{$r$ Affects Experiment Incentive}    
  \label{fig:r}            
\end{figure}


$r$ here stands for the patience of the decision maker, hence more efficient experiment will be allowed when he is more patient. The decision whether to switch from Full Coverage to Partial Coverage seems like a myopic decision since $\underline \alpha_3$ is not affected by $r$: the monopolist stops selling risky arm and starts to sell safe arm when risky arm makes less profit. However, it's actually not the case. As we have mentioned before, Partial Coverage has the same learning speed with Full Coverage. Switching to Partial Coverage will not slow down the speed of learning the state, hence $r$ will not affect the switching belief here.







==> chapters/EQ.tex <==
\section{Equilibrium Analysis}
\label{Section_Discrete_Analysis}
This section is organized as follows. In Section \ref{Section_preliminary_analysis} we try to do some preliminary analysis for the optimal bonus scheming problem where some definitions are declared, and the key conclusion is that the possible optimal strategy is one of the following strategies: Non Bonus, Immediate Revelation, Recursive Partial Coverage and Recursive Full Coverage. In Section \ref{Section_optimal_FC_PC} we discussed the optimal solutions under these different strategies (mainly for FC and PC) in both a finite setting and an infinite setting. Though the process of solving the finite case and infinite case is different, the results are highly similar. In Section \ref{Section_optimal_scheme} we describe the optimal bonus-pricing scheme and try to do some explanations for some economics insights.

\subsection{Preliminary Analysis}
\label{Section_preliminary_analysis}
Define $t_0\equiv\min\{t|\text{ agent } t \text{ reports } R_1\}$.
Then firstly the monopolist can make $t_0\ge T$ by setting $b_t=0, \forall t$, and sell safe arm or risky arm respectively by setting $p_1=\mathbb ER_1,p_2=R_2-\epsilon$ or $p_1=\mathbb ER_1,p_2=R_2+\epsilon$. In this case all the agents purchase the corresponding arm but no information revelation are achieved. We call these two corner solutions as ``Safe Arm'' strategy and ``Non Bonus'' strategy respectively\footnote{The monopolist can also make $t_0=1$ by setting either $b_{1}=\bar c$ and $p_{1,1}=\mathbb ER_1$ or $b_{1}>\bar c$ and $p_{1,1}= \mathbb ER_1+b_{1}-\bar c$. In this case the first agent will purchase arm 1 and report $R_1$ for sure. Hence we denote this strategy as ``Immediate Revelation''. We assume this stretegy out in formal context and leave it to Appendix \ref{Section_IR}}. 

Then given $1<t_0<T$, there are still two possible strategies. Agent $t_0$ will purchase the risky arm and agents after $t_0$ purchase the optimal arm for sure. But which arm will agents before $t_0$ purchase? Notice that when $R_1$ is unknown, agent $t$ has to choose among purchasing arm 1 and report, purchasing arm 1 and don't report, and purchasing arm 2 given $\{p_{1t},p_{2t},b_{t}\}$. It is straightforward to see that there are two cutoffs $\tilde r_t$, $\tilde r_t'$ such that agent $t$ will choose arm 1 if $c_{t}\leq \tilde r_{t}$ and report $R_1$ if $c_{t}\leq \tilde r_{t}'$.  Then according to this definition we must have 
\[\mathbb E R_1 -p_{1t}+\max\{b_t-c_t,0\}\ge R_2-p_2, \quad \forall c_t \le \tilde r_t\]
and 
\[b_t=r_t'\]
If we set $\tilde r_t'<\tilde r_t$ then we must have $b_t-c_t<0$ and set $p_1=\mathbb E R_1$. In this case, every buyer purchases arm 1, and only those with $c_t<\tilde r_t'$ reports $R_1$. 

On the other hand, if we set  $\tilde r_t'>\tilde r_t$, then we have $p_{1t}=\mathbb E R_1+\tilde r_t'-\tilde r_t$. In this case, only those buyers with $c_t<\tilde r_t$ purchases arm1, but they will report $R_1$ for sure after purchasing.

In the first case, $t_0=\min\{t|b_t\geq c_t\}$. Before $t_0$, the platform sells arm 1 at price $\mathbb ER_1$ but does not pay any bonus. At $t_0$, the platform gets $p_{1t}-b_{t}=\mathbb ER_1-b_{t_0}$. So given $t_0$, the utility of the platform is:
\begin{equation}
(1+r+...+r^{t_0-1}) \mathbb E R_1+(r^{t_0}+r^{t_0+1}+...+r^{T-1})\mathbb E \max\{R_1,R_2\}-r^{t_0-1} b_{t_0}.\label{equation_1} 
\end{equation}

In the second case, similarly we have $t_0=\min\{t|\mathbb ER_1+b_{t}-p_{1t}\geq c_t\}$. Before $t_0$, the platform sells arm 2 at price $R_2$ and at $t_0$, the platform gets $p_{1t}-b_{t}=\mathbb ER_1-b_{t_0}$. So the platform gets:
\begin{equation}
(1+r+...+r^{t_0-2}) R_2+r^{t_0-1} \mathbb E R_1+(r^{t_0}+r^{t_0+1}+...+r^{T-1})\mathbb E \max\{R_1,R_2\}-r^{t_0-1} b_{t_0}.\label{equation_2}
\end{equation}

Hence before the information of $R_1$ is revealed ($t_0$), the monopolist can either sell risky arm for every agent, or sell safe arm but set a bonus to motivate someone to explore the risky arm (In our Appendix A we proved that mixing these two strategies will never be optimal). We denote these two strategies as ``Full Coverage'' and ``Partial Coverage'' strategy respectively.  By saying ``selling the certain arm'' we mean the monopolist can guide all the agents to purchase the risky arm by pricing $\epsilon$ lower for the corresponding arm.

 $t_0$ is a description of equilibrium output instead of the equilibrium strategy. After $t_0$ the game is trivial since the monopolist will sell the arm with the highest utility. The following definitions are only for strategies that may be equlibirum strategies:
\begin{definition}
	~\\
	\begin{enumerate}
	    \item The platform uses ``Non Bonus'' Strategy (NB) if the platform sets  $b_t\le 0, \forall t\le T$ and keeps selling the risky arm forall $t\le T$. 
	    \item The platform uses ``Safe Arm'' Strategy (SA) if the platform sets  $b_t\le 0, \forall t\le T$ and keeps selling the safe arm forall $t\le T$. 
	    \item The platform uses ``Full Coverage'' Strategy (FC) if the platform sets $b_1\in (0,\bar c)$ and keeps selling the risky arm before $t_0$.
	    \item The platform uses ``Partial Coverage'' Strategy (PC) if the platform sets  $b_1\in (0,\bar c)$ and keeps selling the safe arm before $t_0$.
	    \item The platform uses ``Immediate Revelation'' Strategy (IR) if the platform sets  $b_1\ge \bar c$. 
	\end{enumerate}
 \label{definition}
\end{definition}
There are two points to note. Firstly we should explain the difference between FC and PC. 
 Under Full Coverage Strategy, the platform always sells arm 1 before $R_1$ is revealed but the value of $R_1$ may not be reported. Under Partial Coverage Strategy, the platform sells both arm 1 and arm 2 before $R_1$ is revealed, and the value of $R_1$ is always revealed after an agent purchases arm 1. Though in definition we call a selling strategy Partial Coverage whenever the platform sells the safe arm at least once, we prove in Appendix that it's not optimal for the platform to mix between these two arms: in the equilibrium path, the seller either keeps selling risky arm until one consumer reports, or he keeps selling safe arm until one consumer purchases the risky arm and reports its utility.
 

 
 Secondly it's natural to treat NB as corner solutions of FC when $b_t\equiv 0$, and treat SA as corner solutions of PC when $b_t\equiv 0$.  Here we tell them apart to make things clear. Using the NB strategy means that the platform believes that the expected utility of the risky arm is high enough that it does not need to reveal information to further increase the pricing, while using the SA strategy means that the platform believes that the risky arm is not comparable to the safe arm, and the  information is not worth revealing since it's too costly.  
 IR can also be treated as a corner solution of both FC and PC by setting $b_1=\bar c$. And using IR means the platform values this information a lot and wants to reveal it as soon as possible even with a very high cost.

 For the subsequent analysis, we declare some notations here:
\[M=\mathbb Emax\{R_1,R_2\}-\mathbb ER_1\]
\[N=M+\frac{\mathbb E R_1-R_2}{r}\]
\[\beta(x)=\frac{H(x)}{h(x)}+x,x\in[0,\bar c]\]
\[\psi(x)=\left\{
\begin{aligned}
	&\beta(x)+M-\frac{H^2(x)}{h(x)}& \text{ if } x\in[0,\bar c]\\
	& x+M &\text{ otherwise }
\end{aligned} \right.\]

\[\psi_N(x)=\left\{
\begin{aligned}
	&\beta(x)+N-\frac{H^2(x)}{h(x)}& \text{ if } x\in[0,\bar c]\\
	& x+N &\text{ otherwise }
\end{aligned} \right.\]
\[\Psi(x)=(1-\frac{1}{r})\beta(x)+M-\frac{H^2(x)}{h(x)}\]
\[\Psi_N(x)=(1-\frac{1}{r})\beta(x)+N-\frac{H^2(x)}{h(x)}\]

Finally we denote \[\Gamma(x)=\beta^{-1}(r\psi(x))\] and \[\Gamma_N(x)=\beta^{-1}(r\psi_N(x))\] for the recursive equation of bonus, and we let $b^*,b_N^*$ stand for the fixed point of $\Gamma(\cdot),\Gamma_N(\cdot)$ respectively. We can get some immediate mathematical results based on Assumption \ref{Inada} and \ref{assumption:monotone_beta}:
\begin{enumerate}
	\item there exists $b^*$ if $M<(\frac{1}{r}-1)\bar c+\frac{1}{rh(\bar c)} $ \footnote{If this condition is not satisfied, the iteration relationships in Lemma \ref{FC_lemma_finite} shows for any $b_{p+1}$ we should set $b_p>\bar c$, hence an direct conclusion is that the Immediate Revelation is always optimal when $M>(\frac{1}{r}-1)\bar c+\frac{1}{rh(\bar c)} $. To avoid too much discussion on this trivial case, we can define $b^*=\infty$ for consistency in this case, since it doesn't matter in Proposition  \ref{FC_proposition_finite}.}. 
	\item if $b^*$ exists, it's unique and positive.
\end{enumerate}

Similar results about $b_N^*$ can be found in Appendix Fact \ref{PC_fact_signal} and \ref{PC_fact_sequence}. 

According to our Definition \ref{definition} there are five possible optimal strategies in the equilibrium. In order to focus our analysis on the parts relevant to FC and PC, we ignore the possibility of IR in the main text and take care of IR in Appendix 
\ref{Section_IR_discrete_statement}.  The following assumption requires a large enough $\bar c$ in order to rule out the case when Immediate Revelation is optimal. Assumption \ref{assumption_exist_bstar} also guarantees the existence of $b^*$.
\begin{assumption}
	$\Psi(\bar c)<0$ and $\Psi_N(\bar c)<0$
 \label{assumption_exist_bstar}
\end{assumption}
In the following analysis we consider four different strategies: FC and PC, and their corresponding corner solutions NB and SA.


\subsection{Optimal Solutions under Different Strategies in Finite Case}
\label{Section_optimal_FC_PC}
In Section \ref{Section_optimal_FC_PC}, we consider the cases of finite cases (i.e. $T<\infty$) and infinite cases (i.e. $T=\infty$) simultaneously. 
Though strictly speaking the proof process is different, our results show a highly similarity of solutions under different strategies or different cases. 

\subsubsection{Full Coverage Strategy (including corner case Non Bonus)}

In the full coverage case, holding price for arm 2 $R_2$, the optimal price of arm 1 is always $\mathbb ER_1-\epsilon$ before $R_1$ is fully revealed to guide consumers to purchase arm 1. So we only need to characterize the optimal bonus scheme. The following lemma is the first step of fully characterizing the optimal solution to maximization problem generated by equation (\ref{equation_1}):
\begin{lemma}
	Suppose that there exists $1\leq p<T$ such that the corresponding optimal bonus scheme satisfies $b_{p+1}<b^*$. Then we have the following recursive relationship for any $1\leq T\leq +\infty$:
	\begin{equation}
		b_p=\Gamma(b_{p+1}),\label{recurrence}
	\end{equation}
	where $M=\mathbb Emax\{R_1,R_2\}-\mathbb ER_1$ and $\psi(\cdot)$ as denoted ahead. Given $0<b_{p+1}<b^*$, the solution of equation \ref{recurrence}, $b_p$ exists and $b_{p+1}<b_p<b^*$  
 \label{FC_lemma_finite}
\end{lemma}

Lemma \ref{FC_lemma_finite} actually describes the necessary condition of a recursive (interior) bonus scheme when using Full Coverage strategy. In the proof process we can find that the results shown in Lemma \ref{FC_lemma_finite} does not depend on $T<\infty$ or not.
The monotonicity of above functions guarantees the existence and uniqueness of the solution $b_p$ given $b_{p+1}$. It also guarantees the existence and uniqueness of the fixed point, $b^*$, which is the root of $\Psi(x)$. Actually equation (\ref{recurrence}) defines an iteration constructed by monotone increasing function:
\[
b_p=\Gamma(b_{p+1})\equiv \beta^{-1}(r*[\beta(b_{p+1})+M-\frac{H^2(b_{p+1})}{h(b_{p+1})}])
\]
 Moreover, Lemma \ref{FC_lemma_finite} implies that the optimal interior bonus for agent $p$ only depends on agent $p+1$'s bonus plan in the backward induction sense. Therefore,  the platform's optimal bonus scheme is time consistent, i.e., if the platform designs the optimal bonus scheme at period $p$, the optimal solution should be the same as the initial commitment solution.

Here we characterize the optimal bonus scheme where $T<\infty$. The recursive relationship given in Lemma \ref{FC_lemma_finite} allows us to use a backward induction procedure to calculate the optimal bonus scheme. First of all, it is easy to see that $b_T=0$ since the platform no longer care about the knowledge of $R_1$ when no agent is left. Then, Equation (\ref{recurrence}) allows us to solve the optimal bonus scheme $b_t$ backwardly. Assumption \ref{assumption_exist_bstar} allows us to rule out the corner solution when $b_t>\bar c$, and the following proposition describes the optimal FC strategy. 
\begin{proposition}
Under our Assumption \ref{Inada}, Assumption \ref{assumption:monotone_beta} and Assumption \ref{assumption_exist_bstar}, the optimal Full Coverage (containing Non Bonus) strategy is to set:

	If $T=1$, the optimal full coverage strategy is to set $b_1=0$ (degenerates into corner solution NB)
	
	For $\forall T\ge 2$, NB is never optimal. Construct the sequence $\{b_t\}$ as follows:
	\begin{enumerate}
		\item  if $T<\infty$, let $b_t=\Gamma^{(T-t)}(0)$ for $1\le t\le T$.
		\item  if $T=\infty$, let $b_t=b^*$ for $1\le t\le T$ ($b^*$ is the fixed point of function $\Gamma(\cdot)$ as declared in section 4.1).
	\end{enumerate}
 \label{FC_proposition_finite}
\end{proposition}

Proposition \ref{FC_proposition_finite} shows the algorithm of optimal bonus structure in finite case. Sequence $\{d_t\}$ reveals the recurrence structure of the bonus scheme (recursive FC).  If $T\ge 2$, $d_1$ is positive for sure since $d_1$ is the result of $T-1$ times of increasing iteration starting from 0, hence we do not need to concern whether $d_1\le 0$ in this case. In other words, information about $R_1$ is always worth exploring as long as there is left agents. Or equivalently, NB is always dominated by the optimal FC when $T\ge 2$.

 Results in infinite case are also presented in Proposition \ref{FC_proposition_finite}. Different from finite case, we can not exert backward induction, hence we have to perform the induction from the beginning by using  $b_{p+1}=\Gamma^{-1}(b_p)$ given in Lemma 4.2. The existence and the uniqueness of $b_p$ given $b_{p-1}$ can be inherited from Equation (\ref{recurrence}).  A constant bonus scheme is intuitive given the fact that the platform faces the same designing condition and the same stage game where ever the game starts. Still, we know the fixed point here is positive and unique, which means the intuition before still holds.



\subsubsection{Partial Coverage Strategy (including corner case Safe Arm)}
If the platform chooses partial coverage strategy, he sells the safe item before $R_1$ is revealed. In other words, the platform will optimally set $p_2=R_2$, $p_1=\mathbb ER_1+\epsilon$, hence for agents whose $c_t>b_t$, he purchases $R_1$ get surplus $-\epsilon<0$ hence he will choose $R_2$. But for agents $c_t<b_t$, he will still choose $R_1$ and get surplus $\mathbb ER_1+b_t-c_t-p_1$. We should notice that $p_1-b_t$ will always be shown as a part, hence we can set any $p_1>\mathbb ER_1$ and make $b_t$ an upward translation with equal distance. Hence in the following analysis we just set $p_1=\mathbb ER_1+\epsilon$ and let $\epsilon \to 0^+$. The mathematical structure is similar to Full Coverage case, and Lemma \ref{PC_lemma_finite} (omitted here) is similar to \ref{FC_lemma_finite} which describes the recursive structure of possible optimal strategies.

\begin{proposition}
	For $\forall T\ge 1$, construct the sequence $\{d_t\}$ as follows:
	\begin{enumerate}
		\item  let $d_T$ to be the root of equation $\beta(d_T)=\mathbb ER_1-R_2$
		\item  if $T<\infty$, let $d_t=\Gamma_N^{(T-t)}(d_T)$ for $1\le t\le T$.
		\item  if $T=\infty$, let $d_t=b_N^*$ for $1\le t\le T$ ($b_N^*$ is the fixed point of function $\Gamma_N(\cdot)$ as declared in section 4.1).
	\end{enumerate}
 Under our Assumption \ref{Inada}, Assumption \ref{assumption:monotone_beta} and Assumption \ref{assumption_exist_bstar}, the optimal Partial Coverage (including Safe Arm) strategy is to set:
	\begin{enumerate}
		\item  $(b_{N1},b_{N2},...b_{NT})=(d_1,d_2,...d_T)$, if $0\le d_1$  (PC).
		\item $(b_{N1}=0,b_{N2}=0,b_{N3}=0,..b_{NT}=0)$ if $d_1<0$ (SA).
	\end{enumerate}
   \label{PC_proposition_finite}
\end{proposition}

The bonus scheme is almost the same despite that the platform may have a negative $d_1$ in the iteration sequence. The reason is that the starting point of the iteration, $d_T$ may be negative, unlike in Full Coverage Strategy where $d_T=0$ for sure. This phenomena is a key difference in PC and FC.  Intuitively, a negative $d_1$ shows that the platform acts as if it's ``punishing'' consumers who purchase arm 1, though it's not realistic since consumers can always purchase arm 1 and leaves no feedback to avoid this negative bonus. However, it seems that this is the best the platform can do in order to de-motivate consumers from buying arm 1. Actually, it's equivalent to set $(0,0,0...0)$ and set $p_1=\mathbb ER_1+\epsilon$ and $p_2=R_2$ to guide consumers to purchase arm 2. A straightforward explanation is, in this case, the platform do not want any consumers to purchase from arm 1. Though knowing the exact value of $R_1$ is beneficial, it may not be worthwhile to let one consumer to exploit arm 1, meaning the platform has to bear the expected loss $R_1-\mathbb ER_1$ to do so. In other words, recursive Partial Coverage (PC) may  degenerate into Safe Arm (SA) in this case.

As for the infinite case, a certain problem occurs. It's possible that the fixed point in PC, $b_N^*$, may be negative. Actually,  $b_N^*$ is the root of the following equation: 
\begin{equation}
	(\frac{1}{r}-1)[\frac{H(x)}{h(x)}+x]+\frac{H^2(x)}{h(x)}=N,\label{Actual}
\end{equation}
Obviously, the left hand side of Equation \ref{Actual} is monotonically increasing with respect to $x$, hence it values from 0 to $(\frac{1}{r}-1)[\frac{1}{h(\bar c)}+\bar c]+\frac{1}{h(\bar c)}$. Hence when $N<0$, using the interior expression of $H(\cdot)$ results in a negative $b_N^*$. Hence we say in this case we have $b_N^*<0$, by which we mean Equation \ref{Actual} has no reasonable solution in interval $[0,\bar c]$ since $N<0$.




\subsection{Optimal Bonus Scheme}
\label{Section_optimal_scheme}
To find out the optimal bonus scheme, we calculate the payoffs first. We have the following lemma, whose illustration is in Figure \ref{3totalUR2}. 
\begin{lemma}
For $\forall 0\le T\le \infty$	if $b_1$ and $b_{N_1}$ both lie in $[0,\bar c]$, then:\\
\[\pi_L=\left\{
\begin{aligned}
	&\mathbb E\max\{R_1,R_2\}\frac{1-r^T}{1-r}-\psi(b_1)& \text{ if } L=\text{Full Coverage}\\
	&\mathbb E\max\{R_1,R_2\}\frac{1-r^T}{1-r}-\psi(b_{N_1})& \text{ if } L=\text{Partial Coverage}\\
	&R_2\frac{1-r^T}{1-r} &\text{ if } L=\text{Safe Arm}\\
	&\mathbb E R_1\frac{1-r^T}{1-r} &\text{ if } L=\text{Non Bonus}
\end{aligned} \right.\]
\label{optimal_lemma}
\end{lemma}

We use Figure \ref{3totalUR2} as a numerical illustration\footnote{In this numerical case we assume $T=3,\bar c=1.1,r=0.95, R_1\sim U[0,4]$, hence $\mathbb ER_1=2$. We let $R_2$ ranges from 1.1 to 3.1 hence the max possible $M$ values around 1.2 (in this case $M=\frac{R_2^2}{8}$). $\Psi(\bar c)\le -0.166<0$, and $\Psi_N(\bar c)<0$ since $N<0$ in this case. Hence Assumption \ref{assumption_exist_bstar} is always satisfied. }. The illustration shows  FC tends to NB when R2 is low enough, and PC tends to SA when R2 is high enough. In other words, there exists cutoffs of $R_2$ such that SA dominates PC when $R_2>\hat R_2$, and PC dominates FC when $R_2>\bar R_2$. Given the explicit expression of our Lemma \ref{optimal_lemma}, we know $\bar R_2=\mathbb ER_1$ at which FC=PC and SA=NB. $\hat R_2$ is the cutoff when $b_{N1}=0$ where PC=SA. Moreover we have $\hat R_2>\bar R_2$ given $T\ge 2$ for sure since $R_2=\bar R_2$ leads to $b_{NT}=0$ and therefore a positive $b_{N1}$. When Assumption  \ref{assumption_exist_bstar} fails, i.e. we have to consider the Immediate Revelation case, an illustration and analytical solution can be found in Appendix \ref{Section_IR_discrete_statement} with Figure \ref{3totalUR2T8pic} and \ref{3totalUR2T8barc01pic}. When $T\to \infty$ the similar illustration can be found in Figure \ref{u_R2_infty}.

\begin{figure}[H]
	\centering
	\includegraphics[width=0.5\linewidth]{figures/FC_PC_SA_NB.png}
	\caption{Profit-$R_2$ Under Different Strategies }
	\label{3totalUR2}
\end{figure} 

Given Lemma \ref{optimal_lemma}, then the following proposition is quite clear:
\begin{proposition} Under our Assumption \ref{Inada}, Assumption \ref{assumption:monotone_beta} and Assumption \ref{assumption_exist_bstar},
	if $T\ge 2$, there exists two cutoffs of $R_2$: $0<\bar R_2<\hat R_2$ such that 
	\begin{center}
		The optimal selling strategy is FC if $0<R_2<\bar R_2$\\
		The optimal selling strategy is PC if $\bar R_2<R_2<\hat R_2$\\
		The optimal selling strategy is SA if $\hat R_2<R_2$\\
	\end{center} 
	If $T=1$, there exists one cutoff of $R_2$: $0<\bar R_2$ such that 
	\begin{center}
		The optimal selling strategy is NB if $0<R_2<\bar R_2$\\
		The optimal selling strategy is SA if $\bar R_2<R_2$\\
	\end{center} 
 \label{optimal_proposition}
\end{proposition}

Proposition \ref{optimal_proposition} concludes the optimal strategy when we can ignore IR. And it works for both $T<\infty$ and $T=\infty$. Then we emphasize some trade offs here.
\subsubsection{Partial Coverage v.s. Full Coverage}
We should point out the key difference between FC and PC strategy and we take the finite case as an example. The starting point of backward induction may be different. In FC case, arm 1 is always purchased no matter whether the bonus is taken, hence by backward induction the starting point is always setting $b_T=0$. But in PC case, if the bonus is not taken, arm 2 will be purchased. Hence when $R_2$ is extremely small the platform would have motivation to set some bonus for agents to purchase arm 1 even when he is the only one agent left and information of $R_1$ is of no value. Otherwise when $R_2$ is extremely large, the platform may prefer not to motivate agents to purchase arm 1 by setting zero bonus, and that's the reason why Safe Arm strategy appears. Figure \ref{3totalUR2} describes this insight, since we can find that when $R_2$ is small, FC dominates PC, and when $R_2$ is large, PC is more attractive (the platform will decrease the bonus to 0 when $R_2$ is large enough, which is the when PC degenerates into SA).

A seemingly surprising conclusion is that, in both strategies the $t_0$ has the same expectation value. Though it seems that in PC we define $t_0=\min\{t|c_t<r_t+\mathbb ER_1-p_1\}$, but in equilibrium the platform will increase the bonus for the agent to compensate the utility loss $p_1-\mathbb ER_1$ for agents hence no matter how large $p_1$ is, it will be return back in form of bonus. Hence in our equilibrium analysis we directly fix $p_1=\mathbb ER_1$. In other words, the motivation to encourage information (which is revealed by $b_i$ and accordingly, $\mathbb E t_0$), is only affected by $\mathbb E\max\{R_1,R_2\}-\max\{\mathbb E R_1,R_2\}$, hence the $\mathbb E t_0$ is the same no matter we use PC or FC. 


Fix $\mathbb ER_1$ and let $R_2$ increase rapidly, from Figure \ref{3totalUR2} we can see there are two important thresholds for $R_2$. 

The first one is $\tilde{R}_2=\mathbb ER_1$ or 2.0 in Figure \ref{3totalUR2}. At this point $\mathbb ER_1=R_2$,$M=N$, and $b_{T}=0$ in PC case. When $R_2<\mathbb ER_1$, we know if the platform insists on using PC we have $\beta(b_T)=\mathbb ER_1-R_2>0$, which means the platform would still like to use a positive bonus to encourage the last agent to purchase arm 1 even there is only one agent left. Hence it's obviously dominated by FC, a more direct way to guide agents purchase arm 1. Hence $\forall R_2 \in [0,\mathbb ER_1]$, the platform should use Full Coverage Strategy\footnote{strictly speaking, Full Coverage and Non-Bonus dominates Partial Coverage and Safe Arm.}. When $R_2>\mathbb ER_1$, in both strategies reporting agent get $\mathbb ER_1$ and yields the same profit. But agents who arrives before $t_0$ and does not report will get $R_2$ in Partial Coverage instead of $\mathbb ER_1$ in Full Coverage. Hence when $R_2>\mathbb ER_1$ the platform should use Partial Coverage Strategy. 

The second one is $\hat{R}_2$ which makes $N=0$ or 3.26 in Figure \ref{3totalUR2}. At this point $N=0$ and $b_N^*=0$. When $R_2>\hat{R}_2$, $N<0$ hence the interior solution sequence $\{b_t\}$ can never be positive (see Figure \ref{bTnegNneg}. More details can be found in Appendix \ref{section_proof_proposition_4_4}). Hence the total bonus structure is equivalent to $(0,0,...0)$, meaning the RPC completely degenerates into a safe arm structure. When $\tilde{R}_2<R_2<\hat{R}_2$, though $b_T$ is negative, the interior solution sequence $\{b_t\}$ may finally get positive since $b_N^*>0$ (see Figure \ref{bTneg}), meaning that when there are still enough agents left the platform should use a positive bonus to encourage reporting, otherwise it will set a zero (negative is equivalent to zero) bonus to prevent loss of $R_2-\mathbb ER_1$ caused by reporting.

\iffalse
Here we should notice that if RM could be optimal, we need $\underline{R}_2>\bar R_2$ (see Figure \ref{3totalUR2T8barc01pic}). Otherwise it's always dominated by RPC or RFC (see Figure \ref{3totalUR2}). A larger $T,r$, smaller $\bar c$ may provide more support for IRM to be optimal according to above insights. A numeric example is provided in our Appendix A.4 where $T=2$.
\fi

\subsubsection{Finite v.s. Infinite}
The platform's optimal selling strategy and bonus method in infinite case are also contained in the corresponding propositions or lemmas, though simply taking the limit is not strict though it yields the right answer and it's more straightforward. Hence in the Appendix \ref{section_proof_proposition_4_3} and \ref{section_proof_proposition_4_4} we focus on the proof of finite cases, and all the proof in infinite cases are placed in Appendix \ref{section_proof_total_utility} since they are based on a different solving process.

Mathematically speaking, the only difference between finite case and infinite case is the discrimination condition of corner solution. In finite case, take FC as an example, we construct sequence $\{d_t\}$ and use  $d_1=\Gamma^{(T-1)}(0)$ to compare with $\bar c$ for corner solution. In infinite case, we use $d^*$, which is the fixed point of the iteration equation and can be understood as $d^*=\Gamma^{(\infty)}(0)$. When $T=\infty$, our insights before may be better understood because the discrimination conditions and the bonus can be expressed explicitly. We provide a numerical illustration in Figure \ref{u_R2_infty}.
\begin{figure}[H]
		\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[scale=0.5]{figures/inf_utility.png}
		\caption{Profit-$R_2$ When $T=\infty$}
		\label{u_R2_infty}
	\end{minipage}
	\begin{minipage}[t]{0.5\linewidth}
		\centering
		\includegraphics[scale=0.5]{figures/inf_bonus.png}
		\caption{Bonus-$R_2$ When $T=\infty$}
		\label{bstar_R2_infty}
	\end{minipage}%
\end{figure}


\subsubsection{$R_2$ and $\mathbb ER_1$ Are Not Enough to Pin Down Everything}
\label{rhosection}
One may think our results are trivial since we are simply comparing $R_2$ and $\mathbb ER_1$ for choosing FC and PC. However we have to point out that fixing $R_2$ and $\mathbb ER_1$, the optimal bonus strategy will not be fixed accordingly. The reason is that the gap between $\mathbb E\max\{R_1,R_2\}$ and $R_2$ will affect the incentive to motivate social learning under Partial Coverage. The same logic works for the Full Coverage region. We may have different $\mathbb E\max\{R_1,R_2\}$ even though we pin down $\mathbb ER_1$ and $R_2$. A simple example can be constructed as follows. We assume $R_1=\rho x+(1-\rho) y$ where $\rho\in(\frac{3}{4},1)$ is a given constant, $x\sim U(0,4)$ and $y\sim U(1,3)$. Let $R_2=3$ then we can calculate $\mathbb E\max\{R_1,R_2\}$
explicitly (more details can be found in Section \ref{proof_rho}).


Hence $\mathbb E\max\{R_1,R_2\}$ is continuous, smooth for $\rho\in [0,1]  $, and it's monotonically increasing with respect to $\rho$. As a result, bonus will increase if $\rho$ increases. Hence we should expect bonus will increase no matter the strategy is FC or PC. In this case $R_2=3>\mathbb ER_1=2$, hence we should use PC. Instead, if we set $R_2=1$, the calculation should be similar, and we will see the bonus is increasing with respect to $\rho$ in FC, too.
An illustration can be found in Figure \ref{rho_affects_bonus}.
\begin{figure}[H]
    \centering
    \includegraphics[width=0.5\linewidth]{figures/rho_affects_bonus.png}
    \caption{$\rho$ Affects Bonus}
    \label{rho_affects_bonus}
\end{figure}



\newpage


==> chapters/Model.tex <==
\section{Baseline Model: Perfect Learning}

In this section, we set up the baseline model in which learning is perfect, i.e. once a consumer reports the utility of the risky arm, it is the exact value. There is a monopoly platform selling two products $i=1,2$ (called arm 1 and arm 2 henceforth) to a sequence of risk neutral agents. The production cost of each arm is normalized to zero. The platform's objective is to maximize its total profit while the agents are maximizing expected utility by choosing one of these two arms.  Each agent receives the same utility from arm $i$ denoted by $R_i$. We assume that the value of  $R_2$ is common knowledge while the value of $R_1$ is unknown both to the platform and to the agents. As in previous literature, arm 2 is called ``safe arm'' and arm 1 is ``risky arm''. Moreover, it is common knowledge that $R_1$ follows a certain distribution $G(\cdot)$. For our further analysis, only the values of $\mathbb ER_1$ and $\mathbb E\max\{R_1,R_2\}$ matter with $\mathbb ER_1<\mathbb E\max\{R_1,R_2\}<\infty.$

A leading example fitting our model very well is the proprietary platform operated by Amazon or JD.com. For the brands sold on such a platform, the platform can either directly determine the price or indirectly affect the price by offering customers coupons or discounts. Moreover, the safe arm corresponds to the well-established big brand for which the customers are quite certain about quality while the risky arm corresponds to the new brand for which both the platform and the customers are uncertain about quality.

Following the social learning literature (see, e.g., \cite{kremer2014implementing}), we assume that there are $T\leq\infty$ agents indexed by the integer $t$. Agents know their positions and take actions in an exogenous order: agent $t$ can make a decision of purchasing in period $t$ only. In our baseline model of perfect learning, an agent can perfectly know the value of $R_1$ after choosing arm 1, and then decides whether to report $R_1$ to the platform. Reporting is costly, and each agent has a private reporting cost $c_i$ distributed in a common support interval $[0,\bar c]$. We assume the distribution function $H(\cdot)$ is strictly increasing and has a smooth density function $h(\cdot)$. Moreover, we impose the following technical assumptions on the density function $h$:
\begin{assumption}
\label{Inada}
The density function $h(\cdot)$ satisfies:
$\lim\limits_{x\to 0^+} h(x)>0$, and  $\lim\limits_{x\to c^-} h(x)>0$.
\footnote{A more general assumption for part 2 in Assumption 3.1 is that there exists some order $p$ such that $\lim\limits_{x\to \bar c^-}h^{(p)}(x)\neq 0$ if $\lim\limits_{x\to \bar c^-}h^{(k)}(x)= 0,\forall k<p$.Here if $\lim\limits_{x\to \bar c^-}h(x)=0$, form L Hospital's Rule $\lambda(\bar c)=M+\bar c+\lim\limits_{x\to \bar c^-}\frac{H(x)-H^2(x)}{h(x)}=M+\bar c-\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ so if $\lim\limits_{x\to \bar c^-}h'(x)=0$ we can still get the same result by using  $\lim\limits_{x\to \bar c^-}h''(x)>0$ or so on. All we need is that the limit $\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ is convergent to zero hence as long as there exist some order $p$ such that $\lim\limits_{x\to \bar c^-}h^{(p)}(x)\neq 0$ if $\lim\limits_{x\to \bar c^-}h^{(k)}(x)= 0,\forall k<p$, which always exists unless $h(x)$ is constant in a neighborhood of $\bar c$. }
\end{assumption}
Technically speaking, these assumptions on the limits are needed because we have to calculate the limit value when $x$ converges to the boundary (in Appendix A.2), and it always holds unless $h(x)$ is constant in a neighborhood of $\bar c$. In economic language, we know the first part of Assumption \ref{Inada} restricts the marginal effect of increasing the size of bonus at the lower bound. The second part also restricts the marginal effect of increasing the size of bonus at the upper bound, since it can be understood as a more general assumption than $\lim\limits_{x\to \bar c^-} h(x)>0$. For example, if $\lim\limits_{x\to \bar c^-}h(x)=0$, from L'Hospital's Rule $\lambda(\bar c)=M+\bar c+\lim\limits_{x\to \bar c^-}\frac{H(x)-H^2(x)}{h(x)}=M+\bar c-\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ so if $\lim\limits_{x\to \bar c^-}h'(x)=0$ we can still get the same result by using  $\lim\limits_{x\to \bar c^-}h''(x)>0$ or so on. All we need is that the limit $\lim\limits_{x\to \bar c^-}\frac{h(x)}{h'(x)}$ is convergent to zero.

Define $\beta(x)=x+\frac{H(x)}{h(x)}$ as the virtue value defined in the mechanism design literature. We impose the standard assumption on $\beta(x)$.
\begin{assumption}
	$\beta'(x)$ is always positive.
 \label{assumption:monotone_beta}
\end{assumption}
In our problem, the platform commits to a sequence of bonuses $\{b_1, b_2,\cdots, b_T\}$ and a sequence of prices $\{p_{i1}, p_{i2}, \cdots, p_{iT}\}$ before the game starts, where $p_{it}$ is the price of arm $i$ for the $t$-th agent if in period $t$ the value of $R_1$ is not revealed, and $b_t$ is the bonus paid to agent $t$ if agent $t$ reveals $R_1$ and none of the agents before $t$ report to the platform (in perfect learning setting, once $R_1$ is revealed, the platform will no longer need reports). We assume that the agent reveals her true utility if she reports. This assumption is reasonable as there is no incentive for lying since each agent is short-lived in our model.  Each agent has a reservation value of zero. So it is straightforward to set $p_{2t}=R_2$. And once $R_1$ is revealed to the platform, the platform will always sell the arm with higher value and get $\mathbb E\max\{R_1,R_2\}$. The platform's problem is to determine $p_{1t}$ and $b_{t}$ before $R_1$ is revealed. 


